Local Model Feature Transformations

Local learning methods are a popular class of machine learning algorithms. The basic idea for the entire cadre is to choose some non-local model family, to train many of them on small sections of neighboring data, and then to `stitch' the resulting models together in some way. Due to the limits of constraining a training dataset to a small neighborhood, research on locally-learned models has largely been restricted to simple model families. Also, since simple model families have no complex structure by design, this has limited use of the individual local models to predictive tasks. We hypothesize that, using a sufficiently complex local model family, various properties of the individual local models, such as their learned parameters, can be used as features for further learning. This dissertation improves upon the current state of research and works toward establishing this hypothesis by investigating algorithms for localization of more complex model families and by studying their applications beyond predictions as a feature extraction mechanism. We summarize this generic technique of using local models as a feature extraction step with the term ``local model feature transformations.'' In this document, we extend the local modeling paradigm to Gaussian processes, orthogonal quadric models and word embedding models, and extend the existing theory for localized linear classifiers. We then demonstrate applications of local model feature transformations to epileptic event classification from EEG readings, activity monitoring via chest accelerometry, 3D surface reconstruction, 3D point cloud segmentation, handwritten digit classification and event detection from Twitter feeds.

==> local_ODQ_regression/results/long_results.tex <==

\section{Results} \label{section:results}

\subsection{Contrived Data} \label{section:contrivedresults}

In this section we investigate a number of practical issues related to obtaining local modeling with Gaussian Processes, including the stability of features over time, hyperparameter selection, and the interpretation of any extracted features.
 We use these initial investigations to inform the setup for later experiments.

\subsubsection{Stability of Extracted Features} \label{section:stability}

At a very basic level, in order for features extracted from a dataset to provide any meaningful insight into the dataset, they should be non-random, and should vary more-or-less continuously with the time-series under consideration.
 By more-or-less continuously, we note that, for example, change point detection algorithms produce non-continuous output in the form of a point-impulse at various locations.
 However, the number of discontinuities in the signal output by a change point detection algorithm are relatively few, and the output features are almost everywhere 0 (indicating no-change).
 On the other hand, features that consist of a very large number of large jump discontinuities are probably not helpful.
 We note this because the algorithm described in Section \ref{section:algorithm} is not mathematically guaranteed to provide stable output.

However, by experiment we show that, by appropriate choice of hyperparameters and other factors, we can encourage a sufficient amount of stability in the extracted features.
 In the remainder of this section, we will explore the underlying mechanisms which might cause instability in the output of the algorithm, and to then propose ways that we might mitigate these issues.

In general, for kernel methods, a smooth kernel gives a smoothly varying optimization surface at each point in time, which results in a smoothly varying optimum over time.
 However, this helpful property does not apply for us, because of the fact that the optimization surface of a GPR is not generally convex.
 Therefore, our algorithm may exhibit discontinuities depending on a variety of factors.
 These include, but are not limited to the choice of seed for the optimizer at each point in time and the number of parameters available to our chosen covariance function.
 Regardless of how we might choose a seed for our optimizer, or various other considerations, however, the output of the algorithm cannot be guaranteed to be continuous.

Before continuing, we would like to examine the continuity claim above that we would have if the optimization surface \emph{were} convex.
 For mathematical simplicity, we only consider here loss functions of the following form, which is a very common form:
%
\begin{equation}
 L(X,\theta,q) = \sum_{x\in X} l(x,\theta)K(x,q)
\end{equation}
%
 Where $X$ is our dataset of size $n$, $l(x,\theta)$ is a bounded loss for a single point $x$, given parameters $\theta$, and $K(x,q)$ is the weight at point $x$ given a query point $q$.
 We are specifically concerned with local weighting schemes, and we will ask what happens to this total loss as the query point changes by a small amount.
 Suppose then, that we have some small quantity in mind, $\delta > 0$ and that $|l(x,\theta)| < M$.
 If $K$ is continuous and symmetric, then we can choose $\epsilon>0$ so that $|K(x,q')-K(x,q)| < \delta/(nM)$ for a given $x$ whenever $|q-q'|<\epsilon$.
 This implies that $|L(X,q',\theta) - L(X,q,\theta)| < \delta$, so that the total loss is also continuous in $q$ at any given $\theta$.
 Our requirement that $l$ be bounded amounts to a bound on $\theta$, but since our dataset $X$ is fixed, this is not an unreasonable requirement for most model families.
 
We would like to see that the optimal parameters $\theta_\text{opt}(q)$ that minimize the total loss at $q$ are also continuous in $q$.
 Choose another $\delta > 0$.

First, observe that for any $\delta > 0$ we can choose an $\gamma > 0$ so that:
$$ \begin{array}{l}L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 This can be acheived by simply setting $\gamma$ so to be the minimum difference $L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q))$ for all $\theta''$ so that $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 To show the contrapositive, choose a $\theta'$ so that $|\theta' - \theta_\text{opt}(q)| > \delta$.
 Choose $\theta''$ to be the point so that $\alpha \theta' + (1-\alpha) \theta_\text{opt}(q) = \theta''$ where $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 Since $L(X,q,\theta)$ is convex in $\theta$ for a given $q$ then:
$$L(X,q,\theta'') < \alpha L(X,q,\theta') + (1-\alpha) L(X,q,\theta_\text{opt}(q))$$
 This gives:
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) \\ > (L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q)))/\alpha \\ > \gamma/\alpha > \gamma \end{array} $$
 
This shows that all of the points $\theta$ that have a ``small" loss are near the current $q$'s optimum.
 We will now combine this fact with $L$'s continuity in $q$ to acheieve the desired result.
 Pick $\gamma > 0$ so that 
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ 
   \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 Further restrict $\gamma$ so that 
$$ \begin{array}{l} L(X,q',\theta') - L(X,q',\theta_\text{opt}(q')) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q')| < \delta/2 \end{array}$$
 Pick $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ \begin{array}{l} 0 < L(X,q',\theta_\text{opt}(q) - L(X,q,\theta_\text{opt}(q) = \\ |L(X,q,\theta_\text{opt}(q)) - L(X,q',\theta_\text{opt}(q))| < \gamma/2 \end{array}$$
 Further restrict $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ L(X,q,\theta_\text{opt}(q')) - L(X,q',\theta_\text{opt}(q')) < \gamma/2$$
 Combining the previous two facts, we have $|q-q'| < \epsilon$ implies 
$$\begin{array}{l} (L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q))) + \\ (L(X,q',\theta_\text{opt}(q) - L(X,q',\theta_\text{opt}(q'))) < \gamma \end{array}$$
 Since $L$ is optimized at $\theta_\text{opt}$, both of these terms are positive, and we have that $L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q)) < \gamma$.
 This implies that $|\theta_\text{opt}(q) - \theta_\text{opt}(q')| < \delta$, which gives the desired result.

In other words, if the optimization surface is convex, then new time series formed by extracted parameters will be continuous.
 If the model family consists of continuous functions, this will further imply a continuous sequence of predictions, which is why LOESS gives continuous curves.
 However, if the optimization surface is \emph{not} convex, then no such continuity is guaranteed.
 Such discontinuities might occur even if the optimization surface is smooth.
 This means that as our time series progresses, the extracted model parameters may experience discontinuities, and these discontinuities are not necessarily related to anything special happening in the data.
 We show this by counterexample.

In Figure \ref{figure:discontinuousoptimaneighboringbeta0}, we show potential loss surfaces over which we intend to optimize a parameter displayed on the $x$ axis.
 Imagine that, as we change $q$, the optimization surface changes at each time step from the function at top to the function at bottom.
 At the top, the loss surface contains a single minimum, which our optimization procedure finds.
 If we seed a gradient descent optimizer with the previous time steps optimum, we will find the points in red.
 Note that this point changes continuously until the local optimum at that point disappears, at which point the optimizer slides to an entirely new local minimum elsewhere.
 The point at which this local minimum disappears will create a discontinuity in the extracted parameters.
 In the case that we use an optimizer that is capable of finding the global minimum at each point, there will be a discontinuity in the optimum at the middle function ($h=1,k=-1$), at which point the two optima have an equal loss.
 In the case that we use a gradient descent optimizer seeded with a constant value, it will experience a discontinuity, but it is not clear at what point that discontinuity will occur.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_neighbor_beta0}}}
    \caption{The family of functions $3x^4-4(k+h)x^3+6khx^2$ for varying values of $h,k$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the previous time-steps optimum.}
    \label{figure:discontinuousoptimaneighboringbeta0}
\end{figure}

Worse, if we seed a gradient descent optimizer with a constant value, the local optima need not disappear in order to experience a discontinuity.
 In Figure \ref{figure:discontinuousoptimaconstantbeta0}, we can see that such a thing might happen.
 Note that this observation also holds for a robust global optimizer that finds the global optimum.
 In the same figure, the two displayed optima have the same loss value, so that a global optimizer might jump between these two values due to small fluctuations.
 Thus, we expect a good global optimizer to actually give \emph{less} stable results than a simple gradient descent optimizer with an appropriate seed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_fixed_beta0}}}
    \caption{The family of functions $(x-h)^4-2(x-h)^2$ for varying values of $h$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the seed at the orage vertical line.}
    \label{figure:discontinuousoptimaconstantbeta0}
\end{figure}

Lastly, we note that, even if a gradient descent optimizer seeded with the previous time-steps optimum does not experience a discontinuity due to the disappearance of the previous time-step's optimum, the local optimum may become very sub-optimal over time.
 Worse, the series of extracted parameters can therefore become `stuck' at a poor local optiumum, and may remain there for the entire time series.

So, we see that when the optimization surface is not guaranteed to be convex, the extracted features cannot be guaranteed to be continuous.
 However, the strategy by which we seed the optimizer can have an effect on the stability of the results.
 We consider here, empirically, the 3 optimizer strategies discussed above: constant seed, seed with neighboring interval optimum value, and global optimization.

All of these options can be seen in practice in Figure \ref{figure:contrivedvariancevariousfixedparameters}, displaying results from the various seed strategies, and also for various selections for fixing covariance function hyperparameters, which we discuss later in this section.
 In each of the graphs in Figure \ref{figure:contrivedvariancevariousfixedparameters}, the constant term and RBF term parameters are fixed to various values, and the optimizer for the remaining white noise term $w$ is seeded according to various strategies.

In the third set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we simply seed the the optimizer with a starting value that is equal to the fixed constant term value used for that set of features. 
 This seed is employed at every point in time.
 In the 1st and 5th graph down, we can see that some choices of hyperparameters can result in an unstable set of features.
 However, in the 2nd, 3rd and 4th graphs, we can see that a good choice of hyperparameters can result in a more stable set of features.

In the second set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters} we seed the optimizer with the optimum found at the previous point in time.
 We can see in 1st and 3rd graphs that, although the extracted parameters seem to pick up on the change in white noise level, they do not readily return to `normal' levels after the period of altered noise.
 This suggests that they have become `stuck' at a suboptimal local minimum.
 Worse, the 1st, 3rd and 5th graphs suggest that the strategy of seeding the optimizer with a neighboring query point's optimal parameters is not as helpful in encouraging stability as we might have hoped.

In the top set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we seed the optimizer with both the previous time step's optimal parameters and also the exemplar period.
 If the optimum found by seeding with the exemplar parameters has a higher marginal likelihood than at the optimum found by seeding with the neighboring optimum, we fit a GPR with hundreds of seeds spread log-uniformly throughout the parameter space.
 This emulates fitting an optimizer capable of finding the global optimum.
 It is clear that fitting a global optimizer is even more unstable than fitting an optimizer with a fixed seed.
 We suspect that this is because, with a fixed seed, the optimizer can only find local optima "near" the seed.
 However, with a global optimizer, we can find the global optimum no matter where it should appear in the search space, so there is more opportunity for the optimum to switch.
 In any case, it seems that in practice, the global optimizer creates highly unstable results.
 This is just as well, because seeding an optimizer with hundreds of seeds is incredibly time-consuming, and results in a significantly less efficient process.

Furthermore, for various covariance functions and data, the sought-after optimum might be in a very "narrow" valley.
 To the point that finding it using a random seed is a rather unlikely event, and so a great number of seeds must be employed to reliably find good optimal paramter estimates.
 This is illustrated in Figure \ref{figure:contrivedperiodgpr}.
 These parameters are extracted by training over the constant and period paramters and fixing the length scale and white noise parameters in Equation \ref{equation:variableperiodcovariance}.
 100 random seeds are chosen log-uniformly on $[10^{-10},10^{10}]$ and the optimizer is run on each of these, with the best result taken in the end.
 Approximately half of the time, a period on the order of tens is found, which is representative of the approximate period of the local data at that point.
 Figure \ref{figure:contrivedperiodgprsmooth} shows a Nadarya-Watson-smoothed version of the curve in Figure \ref{figure:contrivedperiodgpr}.
 Note that the period generally increases toward the middle of the data, and decreases toward the edge, which is reflective of the properties of the underlying data.
 However, the "correct" optimum can be difficult to find, especially for periodic covariance functions where one might reasonably expect a local minimum at factors of the "true" period.
 The result is unstable local parameters over time.

From these observations, we believe that seeding the optimizer with a fixed set of parameters that are near a "normal operating" value to be a good partial solution to the discontinuity problem.
 The proceeding experiments will therefore all employ this option.

Another strategy that can be employed to increase the stability of the results is to reduce the size of the parameter space.
 Specifically, we would a priori expect that an optimization surface over many variables would have more opportunities to play host to superfluous local optima than an optimization surface over fewer variables.
 One way to accomplish this is by `fixing' some of the parameters in the covariance function at convenient values to allow analysis only of parameters of interest.
 Fixing the parameters of the individual models has other side-effects on the model in addition to affecting the stability of the algorithm.
 It is worth noting that a `fixed' parameter essentially becomes a hyperparameter of the algorithm that must be set by some means besides the ordinary training scheme.
 We therefore discuss these effects in the proceeding section

\subsubsection{Setting Hyperparameters} \label{section:hyperparameters}

Similarly to LOESS or kernel density estimation, we must set a kernel bandwidth.
 There has been a great deal of work into bandwidth selection, with a number of reviews covering the subject, for example \cite{turlach1993bandwidth}.
 The effects of bandwidth selection have mostly been considered in relation to local model predictions.
 However, since predictions are generally a function of the parameters, the sundry factors largely translate to the problem at hand.
 Since our datasets contain relatively little data with which to train this hyperparameter, we set it naively using a priori information concerning the nature of our datasets, and do relatively little to explore its effects.

The remaining hyperparameters consist of any fixed parameters in our covariance functions.
 Fixing the parameters in our covariance function may seem to be a strange step from the point of view of attempting to accurately model the data, so we discuss it briefly here.
 We remind the reader that \emph{our purpose here is not to model the data as accurately as possible}.
 Instead, we aim to extract features from the data for an entirely different purpose than interpolation or extrapolation.
 Therefore, the model most suited to interpolation or extrapolation may or may not be the model best suited to our needs.
 Still, any arbitrary model will not do, and we need a ``well-fit" model in some sense.
 It is important to realize that that sense is some combination of the ordinary sense of fitting models (interpolation and extrapolation) but also the extraction of features best suited for whatever the ultimate use of our features will be.
 Such use cases may include change point detection, as in Section \ref{section:accelerometrymethodology}, time series classification, as in Section \ref{section:eegmethodology} or others.

We note that there are 3 "levels" at which we can allow the various parameters to vary.
 At the highest level, allowing it to vary maximally, we could allow a parameter to be trained in the individual local models.
 At this level, a parameter is simply an additional feature extracted from the time series.
 At a middle level, we could fix the parameter during portions of a sequence, or for a single sequence in a group of sequences, but allow it to vary between sequences
 At the lowest level, we could fix the paramter once for the entire sequence or for all sequences in a group using information gleaned from a set of training sequences.
  
The highest level has the ostensible benefit of providing an additional feature that can be used for learning at a later stage.
 It also benefits from the existence of a pre-existing tried-and-true training method, since they would be obtained from the locally-trained GPRs.
 Lastly, it benefits from the ability to show variation in this parameter between different individuals.
 However, this can result in features that are less stable over time, as the optimizer finds various transient local optima.
 A second pitfall is that the various parameters are not independent.
 In other words, we will obtain a different sequence of white noise term parameters depending on whether we fix the constant term and RBF term parameters or not, and will obtain different sequences depending on what levels we fix them at.
 Both of these problems can be witnessed in Figure \ref{figure:allvarscontrivedvariance}.
 It is therefore not clear that the white noise term sequence will benefit from the additional parameter, and in our experience on this and the accelerometry dataset it does not.

The lowest level solves the problems at the highest level associated with learning multiple parameters.
 It may also help alleviate some of the dependence between parameters during GPR training.
 However it suffers from not allowing variation between individual sequences in a group.
 It is also disadvantaged by ignoring potentially valuable information from an additional extracted feature.
 It also requires the creation of a method for choosing an appropriate fixed parameter.
 However, it is not clear that the additional feature is, in fact, useful: recall the previous discussion concerning the distinction between the best parameters for interpolation vs that for activity recognition.
 If we are specifically interested in one particular parameter, and expect relatively little variation in the scale of other parameters between groups, this option may be best.
 In the third set of graphs of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we can see that this plays out.
 In the contrived variance dataset, although there is some change in, e.g., the curvature of the function over time, which may reflect in the learned parameters, the primary feature of change is the noise level.
 By fixing the other parameters at a convenient level, we can focus the method onto changes in one particular variable, control for the dependence between the parameters, and ease the number of discontinuities in the extracted features over time.
 Specifically, the third graph seems to extract the desired signal from the data very well, giving a large value when the noise level is large, and a small value when the noise level is small.

The middle level also solves the problems at the highest level associated with learning two parameters.
 It also has the benefit of allowing a variation in "baseline" readings between individuals.
 Like the lowest level, it may be disadvantaged by losing an additional feature.
 Similarly, it requires the creation of a method for choosing an appropriate fixed parameter.
 Since the parameter is fixed individually for a sequence, the method devised above for choosing a fixed parameter cannot apply if we cannot depend upon having labelled data for every individual.
 One option may be to train a GPR with the parameter allowed to vary on an exemplar segment of data chosen at random from the sequence, and then to subsequently fix the parameter in the local model training to be the value obtained from the exeplar segment.
 This would solve the problem of optimization surface complexity from the highest level.
 However, it would still suffer from having a parameter chosen for the purpose of interpolation rather than activity recognition.
 Furthermore, there is no guarantee that our `exemplar' segment is, in fact, exemplary.
 Since the contrived data do not involve a great deal of variation in the signal, and do not involve signal from multiple individuals, we do not explore this option here.
 Instead, we include discussion related to this possibility with respect to the accelerometry data, we direct the reader to Section \ref{section:accelerometryresults}, and with respect to the eeg data to Section \ref{section:eegmethodology}.












 Indeed, for this dataset, does an "exemplary" segment come from a sequence where a subject was sitting or walking?
 Still, since it not unreasonable to expect that the best parameter for interpolation might yet be a quite good parameter for other purposes, we investigate this method of setting the constant term parameter as well in Section \ref{section:accelerometerresults}.






Note the length scales of the x-axis in Figure \ref{figure:chestaccelerometerZMinutes}.
 Although the signal appears to have a very prominent noise component when viewed at a resolution on the order of minutes, it is significantly less noticeable when we zoom in to see changes at the level of seconds, as seen in Figure \ref{figure:chestaccelerometerZSeconds}.
 This is because there is meaningful small-scale structure to the accelerometer readings.
 However, that small-scale structure is not necessarily useful in distinguishing between various activities.
 In fact, note that the data in Figure \ref{figure:chestaccelerometerZSecondsfixedrbf} is taken during a single activity, suggesting that a good extracted feature for this data should approximate a constant value indicative of the present activity.
 Allowing the optimizer to choose the parameter of the RBF component of our covariance function may therefore not be an optimal method for extracting the noise component.
 Worse, it is possible for the RBF component to, itself, model white noise.
 Specifically, as the length scale of the RBF component goes to 0, the $CN_c RBF_r$ term simply becomes an $WN$ component.
 It is therefore difficult to prevent interactions between these two terms when optimizing our individual local models.
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr}}}
    \caption{An example taken from the chest accelerometry dataset, showing data on the scale of seconds.
        All parameters in the GPR covariance function (Equation \ref{equation:accelerometergpr}) are allowed to vary.
        400 log-uniform seeds are chosen to obtain globally-optimal parameters.
        The optimal RBF length scale is found to be $\approx 0.33s$.
    }
    \label{figure:chestaccelerometerZSeconds}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr_fixed_r}}}
    \caption{The same data from Figure \ref{figure:chestaccelerometerZSeconds}, but with a fixed RBF length scale parameter at $\approx 15s$
        The remaining parameters are allowed to vary.
    }
    \label{figure:chestaccelerometerZSecondsfixedrbf}
\end{figure}



Since we are primarily interested in the noise level term parameter, we further have the constant term parameter to contend with.
 In Section \ref{section:accelerometerresults}, we provide some exploratory investigation into allowing it full freedom to vary along each time series or fixing it to be a particular value for the entire experiment.
 However, as we have noted, there is a strong interaction between the two additive terms in our covariance function.
 Therefore, we have chosen to fix the constant term parameter as well, at a level convenient for change point detection, chosen by manual inspection of the extracted signals.
 Changing the constant parameter has an effect on the sensitivity of the extracted signal, and also on the stability of the extracted signal.
 Low values give a highly unstable signal.
 High values make the feature extraction insensitive to changes in variance, resulting in a "flat-line" for extremely large values.
 An example set of extracted features, where the hyperparameters are chosen to give a good signal by visual inspection, are seen in Figure \ref{figure:accelerometer5}.
 
Indeed, this is exactly the reason why we fixed the \emph{RBF term} parameter.
 Fixing the constant term parameter, however, is not as straightforward as choosing the RBF term paramter.
 Firstly, the more parameters we fix, the more opportunity there is to constrain our model family in such a way that it cannot possibly give a "good" model.
 Secondly, The units of the RBF term parameter are easily interpretable and therefore lend themselves to being fixed according to our a priori conceptions about the data.
 The optimal constant term parameter is related to the overall variance in the signal, but it also depends on the RBF term parameter, and we therefore lack the insight to simply fix it based on our expertise in the subject.
 Although we cannot set it a priori, it seems reasonable that we might simply train this parameter against a training set of accelerometer readings to optimally predict the true labels.
 We investigate such a procedure in Section \ref{section:accelerometerresults}.





First, there are a number of hyperparameters affected execution of the algorithm.
 Recall from Section \ref{section:accelerometrymethodology} that we have an option to fix various parameters of the GPR during local model training.
 If we elect to fix any of the model parameters, the value at which they are fixed can be considered a hyperparameter of the local model feature extraction.
 Lastly, we need to set the bandwidth for our kernel.
 We will investigate here the effect of all of these various hyperparameters on the results of the algorithm, as well as the effects of fixing the various parameters in the local models.
 Instead of providing a full grid over the various hyperparameters, we will take pick and choose what we consider to be representative possibilities that illustrate possible pitfalls and prospects of local model feature transformations with GPR.

One factor compounding the issue of discontinuous local parameters over time is the dimensionality of the parameter space.
 The larger the space, the more opportunity exists for local optima to appear and disappear, and to generally move up, down and around one another over time.
 Thus, if we identify target parameters that we expect to be indicative of particular properties of interest in our time series, we can potentially "fix" the other parameters.
 This potentially has two advantages.
 First, the size of the parameter space is reduced, potentially improving stability of extracted parameters over time.
 Second, problems with interpreting changes in the local parameters due to dependence between the various parameters is reduced, since only a limited set of the parameters are allowed to vary.
 In other words, changes in a non-target parameter do not cause changes in the target parameter, since the non-target parameter is simply not allowed to vary. 
 We direct the reader to Section \ref{section:accelerometrymethodology} for a more thorough discussion of how "fixing" certain parameters is expected to affect the overall procedure.

Figure \ref{figure:contrivedvariancevariousfixedparameters} shows the results of training a local GPR on our contrived dataset while fixing the RBF term and the constant term's parameters (see Equation \ref{equation:variablevariancecovariance}).
 We seed the white noise parameter with a value of $1$ at all points in time, although we note that the particular seed value used does not much affect the results, so long as the seed is fixed.
 
We will here attempt to explain the extracted features in terms of the intuition behind the chosen form of the covariance function.
 This will provide us with a basis for setting the model parameters in future iterations.
 We note that, although these explanations are based largely on the intuitions outlined in \cite{rasmussen2005gaussian}, they are otherwise post hoc.
 Therefore, these explanations should be taken to be hypothetical.
 Although we will not test them directly, we employ them implicitly in constructing later models, and the reader can weigh the evidence for these explanations in part by the procedure's performance on these subsequent experiments.

 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{illustrative_pairs_contrived_variance}}}
    \caption{Variable noise data below in orange.  
    The three sections divided by a horizontal black line are: top - global parameter search, middle - neighboring parameter seed, bottom - fixed parameter seed.
    Within each section, the graphs in blue represent local GPR white noise parameter freatures obtained with fixed $c,r$ at various values.
    From top to bottom, within each section, the $c,r$ pairs are: $(32,8),(64,2),(64,512),(.25,.12)$ and $(.25,2)$}
    \label{figure:contrivedvariancevariousfixedparameters}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{all_vars_contrived_variance}}}
    \caption{Variable noise data below in pink.
        The other graphs represent the various parameters of a locally trained GPR over time.}
    \label{figure:allvarscontrivedvariance}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr}}}
    \caption{Variable period data below in green.
        Extracted gpr parameters are period for the exponential sine squared term in orange, and the constant term value in blue.
        100 seeds are chosen log-uniformly on $[10^{-10}, 10^{10}]$.}
    \label{figure:contrivedperiodgpr}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr_smoothed}}}
    \caption{The same extracted features from Figure \ref{figure:contrivedperiodgpr}, but smoothed by a weighted rolling mean. 
    }
    \label{figure:contrivedperiodgprsmooth}
\end{figure}


 

\subsection{Accelerometry Data} \label{section:accelerometerresults}

%TODO the transformed data are in chest_acc_run019/transformed_data

In this section we discuss the results of the proposed feature extraction algorithm applied to the accelerometry dataset described in Section \ref{section:accelerometrymethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on discovery of change points in time series.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the signals from 2 different individuals.
 A portion of the signal containing the ground truth change points for both sequences can be seen in Figures \ref{figure:accelerometer5} and \ref{figure:accelerometer6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:accelerometrymethodology} is also shown.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_05_y_axis}}}
    \caption{y-axis acceleration from one of the sequences in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_06_z_axis}}}
    \caption{z-axis acceleration from a second sequence in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer6}
\end{figure}

The hyperparameters used in these graphs were chosen from a log-uniform grid search to return the maximum signal upon visual inspection.
 Although we do not include the full results of the grid search, we refer the reader to Section \ref{section:contrivedresults}, and specifically Figure \ref{figure:contrivedvariancevariousfixedparameters} for comparable results on the contrived datasets.

In Section \ref{section:eegmethodology} we describe a process by which an exemplar model may be used to obtain the seed values for local model training.
 However, this process was not found to be effective for the accelerometry dataset. 



\subsubsection{Confirmatory Results}



\subsection{EEG Epilepsy Data} \label{section:eegresults}

In this section we discuss the results of the proposed feature extraction algorithm applied to the eeg dataset described in Section \ref{section:eegmethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on classification of subsequences of the data.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the positive (including ictal onset) subsamples from 2 different individuals.
 The positive samples contain both ictal and non-ictal activity, and were expected to therefore illustrate the differences in the extracted features for these two types of eeg signals.
 A portion of the signal containing the labeled point of ictal onset for both sequences can be seen in Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:eegmethodology} is also shown.
 Some caution is advised in the interpretation of these graphs, since these are our `training' data, and parameters have therefore been specifically selected in such a way as to obtain a `nice' signal.

Some other configurations of hyperparameters were attempted, but did not give pleasing results.
 Notably, in early experiments we attempted to model the data locally using a covariance function with 4 RBF terms.
 Each was set at a length scale corresponding roughly to the various waveforms commonly encountered in brain activity - beta, alpha, theta and delta waves, and the constant value term was allowed to vary locally.
 However, in experiments, the features extracted at the various length scales were highly correlated, resulting in superfluous features.
 Furthermore, the correlation resulted in a situation where the signal represented by one term overlapped sufficiently with the other terms as to frequently cause a deep local optimum at 0 for the other terms.
 It was therefore often the case that one term would dominate, and the resulting signal was highly unstable with the various terms going to 0 at different times.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00019_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from one of the recordings, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00020_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from a second recording, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset6}
\end{figure}

Due to these issues, the single-term configuration was chosen for improved stability at the expense of interpretability.
 We did not experiment with a wide variety of RBF length scales, since the scale characteristic of theta waves gave reasonable results, and we determined that there was insufficient training data to improve upon that scale by manual inspection or otherwise.
 Although the length scale was fixed at a level representative of theta waves, we expect that variations in the constant term over time will still reflect ratios in the various types of brain waves.
 In Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6} it can be seen that sections of the signal with prominent low-frequency components give high values for the extracted feature, and vice-versa.
 In those same figures, it can be seen that the onset of ictal activity generally seems to involve a move from lower-valued LMFT features to higher-valued ones, although perhaps not in a uniform fashion.
 This observation has informed our hypothesis that the performance of DTW will increase when applied to the LMFT features, since it need only discover the relatively simple transition over time from low to high value, rather than an intricate series of ups and downs associated with the raw eeg signals.

\subsubsection{Confirmatory Results}

Having decided upon a covariance function family and a setting for the various hyperparameters in the exploratory analysis, we proceed to extract features from every channel of every sequence.
 We then employ the validation process as described in Section \ref{section:eegmethodology}.

The confusion matrices for the 3 proposed datasets - raw data, LMFT features and the concatenation of the two - are given in Table \ref{table:eegconfusion}.
 It can be seen that 1NN using DTW for classifying sequences of nonictal eeg activity vs the onset of ictal activity using the raw data is ineffective.
 Indeed, the true label and the predicted label are entirely independent.
 Upon inspection, it seems that 17/19 of the true positive and 15/19 of the true negative validation sequences were matched to two of the training sequences.
 Interestingly, although one of those training sequences was true positive and one true negative, there was no correlation to the label of the validation sequences to which they were matched.
 It is not clear what the cause of this strong preference for certain training sequences was, but the lack of correlation reveals that the raw data are not useful for input directly into a classifier.
 
Similarly, when the raw data and the extracted features were concatenated, 34/38 of the validation sequences were matched to two of the training sequences.
 These two sequences were both negative, and were both different from the two popular sequences from the 1NN with DTW on only the raw data.
 We had expected that the combined information of the raw data and the extracted features would be \emph{more} informative for a classification algorithm, but this did not turn out to be the case.

1NN with DTW on only the LMFT features performed better.
 The gains were modest, giving an accuracy, precision and recall of only 0.66, 0.75 and 0.47 respectively. 
 Still, the intention of the experiment was to show that the LMFT extracted features could be useful for a later classification step, and so these results support our hypothesis.
 We remind the reader that there exist opportunities for training over hyperparamters with larger datasets, and also that the proposed algorithm accepts arbitrary model families.
 This suggests that many improvements to the proposed method might still be made, even for this particular task of epilepsy detection.

\begin{table}[h!]
  \begin{center}
    \caption{EEG classification confusion matrices}
    \label{table:eegconfusion}
    \begin{tabular}{llll|ll|ll}
        &   & \multicolumn{6}{c}{\textbf{Predicted}} \\
        &   & \multicolumn{2}{c}{\textbf{Raw Data}} & \multicolumn{2}{c}{\textbf{LMFT}} & \multicolumn{2}{c}{\textbf{Both}} \\
        &   & -    & +    & -    & +    & -    & +    \\
      \multirow{2}{*}{\textbf{True}}
        & - & 14   & 5    & 16   & 3    & 0    & 19   \\
        & + & 14   & 5    & 10   & 9    & 0    & 19
    \end{tabular}
  \end{center}
\end{table}

%TODO We should go and do a post-hoc analysis on why the misclassified ones were misclassified by viewing the extracted features and seeing what the exemplar model was.


==> local_SVM_projection/results/long_results.tex <==

\section{Results} \label{section:results}

\subsection{Contrived Data} \label{section:contrivedresults}

In this section we investigate a number of practical issues related to obtaining local modeling with Gaussian Processes, including the stability of features over time, hyperparameter selection, and the interpretation of any extracted features.
 We use these initial investigations to inform the setup for later experiments.

\subsubsection{Stability of Extracted Features} \label{section:stability}

At a very basic level, in order for features extracted from a dataset to provide any meaningful insight into the dataset, they should be non-random, and should vary more-or-less continuously with the time-series under consideration.
 By more-or-less continuously, we note that, for example, change point detection algorithms produce non-continuous output in the form of a point-impulse at various locations.
 However, the number of discontinuities in the signal output by a change point detection algorithm are relatively few, and the output features are almost everywhere 0 (indicating no-change).
 On the other hand, features that consist of a very large number of large jump discontinuities are probably not helpful.
 We note this because the algorithm described in Section \ref{section:algorithm} is not mathematically guaranteed to provide stable output.

However, by experiment we show that, by appropriate choice of hyperparameters and other factors, we can encourage a sufficient amount of stability in the extracted features.
 In the remainder of this section, we will explore the underlying mechanisms which might cause instability in the output of the algorithm, and to then propose ways that we might mitigate these issues.

In general, for kernel methods, a smooth kernel gives a smoothly varying optimization surface at each point in time, which results in a smoothly varying optimum over time.
 However, this helpful property does not apply for us, because of the fact that the optimization surface of a GPR is not generally convex.
 Therefore, our algorithm may exhibit discontinuities depending on a variety of factors.
 These include, but are not limited to the choice of seed for the optimizer at each point in time and the number of parameters available to our chosen covariance function.
 Regardless of how we might choose a seed for our optimizer, or various other considerations, however, the output of the algorithm cannot be guaranteed to be continuous.

Before continuing, we would like to examine the continuity claim above that we would have if the optimization surface \emph{were} convex.
 For mathematical simplicity, we only consider here loss functions of the following form, which is a very common form:
%
\begin{equation}
 L(X,\theta,q) = \sum_{x\in X} l(x,\theta)K(x,q)
\end{equation}
%
 Where $X$ is our dataset of size $n$, $l(x,\theta)$ is a bounded loss for a single point $x$, given parameters $\theta$, and $K(x,q)$ is the weight at point $x$ given a query point $q$.
 We are specifically concerned with local weighting schemes, and we will ask what happens to this total loss as the query point changes by a small amount.
 Suppose then, that we have some small quantity in mind, $\delta > 0$ and that $|l(x,\theta)| < M$.
 If $K$ is continuous and symmetric, then we can choose $\epsilon>0$ so that $|K(x,q')-K(x,q)| < \delta/(nM)$ for a given $x$ whenever $|q-q'|<\epsilon$.
 This implies that $|L(X,q',\theta) - L(X,q,\theta)| < \delta$, so that the total loss is also continuous in $q$ at any given $\theta$.
 Our requirement that $l$ be bounded amounts to a bound on $\theta$, but since our dataset $X$ is fixed, this is not an unreasonable requirement for most model families.
 
We would like to see that the optimal parameters $\theta_\text{opt}(q)$ that minimize the total loss at $q$ are also continuous in $q$.
 Choose another $\delta > 0$.

First, observe that for any $\delta > 0$ we can choose an $\gamma > 0$ so that:
$$ \begin{array}{l}L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 This can be acheived by simply setting $\gamma$ so to be the minimum difference $L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q))$ for all $\theta''$ so that $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 To show the contrapositive, choose a $\theta'$ so that $|\theta' - \theta_\text{opt}(q)| > \delta$.
 Choose $\theta''$ to be the point so that $\alpha \theta' + (1-\alpha) \theta_\text{opt}(q) = \theta''$ where $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 Since $L(X,q,\theta)$ is convex in $\theta$ for a given $q$ then:
$$L(X,q,\theta'') < \alpha L(X,q,\theta') + (1-\alpha) L(X,q,\theta_\text{opt}(q))$$
 This gives:
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) \\ > (L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q)))/\alpha \\ > \gamma/\alpha > \gamma \end{array} $$
 
This shows that all of the points $\theta$ that have a ``small" loss are near the current $q$'s optimum.
 We will now combine this fact with $L$'s continuity in $q$ to acheieve the desired result.
 Pick $\gamma > 0$ so that 
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ 
   \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 Further restrict $\gamma$ so that 
$$ \begin{array}{l} L(X,q',\theta') - L(X,q',\theta_\text{opt}(q')) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q')| < \delta/2 \end{array}$$
 Pick $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ \begin{array}{l} 0 < L(X,q',\theta_\text{opt}(q) - L(X,q,\theta_\text{opt}(q) = \\ |L(X,q,\theta_\text{opt}(q)) - L(X,q',\theta_\text{opt}(q))| < \gamma/2 \end{array}$$
 Further restrict $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ L(X,q,\theta_\text{opt}(q')) - L(X,q',\theta_\text{opt}(q')) < \gamma/2$$
 Combining the previous two facts, we have $|q-q'| < \epsilon$ implies 
$$\begin{array}{l} (L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q))) + \\ (L(X,q',\theta_\text{opt}(q) - L(X,q',\theta_\text{opt}(q'))) < \gamma \end{array}$$
 Since $L$ is optimized at $\theta_\text{opt}$, both of these terms are positive, and we have that $L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q)) < \gamma$.
 This implies that $|\theta_\text{opt}(q) - \theta_\text{opt}(q')| < \delta$, which gives the desired result.

In other words, if the optimization surface is convex, then new time series formed by extracted parameters will be continuous.
 If the model family consists of continuous functions, this will further imply a continuous sequence of predictions, which is why LOESS gives continuous curves.
 However, if the optimization surface is \emph{not} convex, then no such continuity is guaranteed.
 Such discontinuities might occur even if the optimization surface is smooth.
 This means that as our time series progresses, the extracted model parameters may experience discontinuities, and these discontinuities are not necessarily related to anything special happening in the data.
 We show this by counterexample.

In Figure \ref{figure:discontinuousoptimaneighboringbeta0}, we show potential loss surfaces over which we intend to optimize a parameter displayed on the $x$ axis.
 Imagine that, as we change $q$, the optimization surface changes at each time step from the function at top to the function at bottom.
 At the top, the loss surface contains a single minimum, which our optimization procedure finds.
 If we seed a gradient descent optimizer with the previous time steps optimum, we will find the points in red.
 Note that this point changes continuously until the local optimum at that point disappears, at which point the optimizer slides to an entirely new local minimum elsewhere.
 The point at which this local minimum disappears will create a discontinuity in the extracted parameters.
 In the case that we use an optimizer that is capable of finding the global minimum at each point, there will be a discontinuity in the optimum at the middle function ($h=1,k=-1$), at which point the two optima have an equal loss.
 In the case that we use a gradient descent optimizer seeded with a constant value, it will experience a discontinuity, but it is not clear at what point that discontinuity will occur.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_neighbor_beta0}}}
    \caption{The family of functions $3x^4-4(k+h)x^3+6khx^2$ for varying values of $h,k$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the previous time-steps optimum.}
    \label{figure:discontinuousoptimaneighboringbeta0}
\end{figure}

Worse, if we seed a gradient descent optimizer with a constant value, the local optima need not disappear in order to experience a discontinuity.
 In Figure \ref{figure:discontinuousoptimaconstantbeta0}, we can see that such a thing might happen.
 Note that this observation also holds for a robust global optimizer that finds the global optimum.
 In the same figure, the two displayed optima have the same loss value, so that a global optimizer might jump between these two values due to small fluctuations.
 Thus, we expect a good global optimizer to actually give \emph{less} stable results than a simple gradient descent optimizer with an appropriate seed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_fixed_beta0}}}
    \caption{The family of functions $(x-h)^4-2(x-h)^2$ for varying values of $h$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the seed at the orage vertical line.}
    \label{figure:discontinuousoptimaconstantbeta0}
\end{figure}

Lastly, we note that, even if a gradient descent optimizer seeded with the previous time-steps optimum does not experience a discontinuity due to the disappearance of the previous time-step's optimum, the local optimum may become very sub-optimal over time.
 Worse, the series of extracted parameters can therefore become `stuck' at a poor local optiumum, and may remain there for the entire time series.

So, we see that when the optimization surface is not guaranteed to be convex, the extracted features cannot be guaranteed to be continuous.
 However, the strategy by which we seed the optimizer can have an effect on the stability of the results.
 We consider here, empirically, the 3 optimizer strategies discussed above: constant seed, seed with neighboring interval optimum value, and global optimization.

All of these options can be seen in practice in Figure \ref{figure:contrivedvariancevariousfixedparameters}, displaying results from the various seed strategies, and also for various selections for fixing covariance function hyperparameters, which we discuss later in this section.
 In each of the graphs in Figure \ref{figure:contrivedvariancevariousfixedparameters}, the constant term and RBF term parameters are fixed to various values, and the optimizer for the remaining white noise term $w$ is seeded according to various strategies.

In the third set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we simply seed the the optimizer with a starting value that is equal to the fixed constant term value used for that set of features. 
 This seed is employed at every point in time.
 In the 1st and 5th graph down, we can see that some choices of hyperparameters can result in an unstable set of features.
 However, in the 2nd, 3rd and 4th graphs, we can see that a good choice of hyperparameters can result in a more stable set of features.

In the second set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters} we seed the optimizer with the optimum found at the previous point in time.
 We can see in 1st and 3rd graphs that, although the extracted parameters seem to pick up on the change in white noise level, they do not readily return to `normal' levels after the period of altered noise.
 This suggests that they have become `stuck' at a suboptimal local minimum.
 Worse, the 1st, 3rd and 5th graphs suggest that the strategy of seeding the optimizer with a neighboring query point's optimal parameters is not as helpful in encouraging stability as we might have hoped.

In the top set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we seed the optimizer with both the previous time step's optimal parameters and also the exemplar period.
 If the optimum found by seeding with the exemplar parameters has a higher marginal likelihood than at the optimum found by seeding with the neighboring optimum, we fit a GPR with hundreds of seeds spread log-uniformly throughout the parameter space.
 This emulates fitting an optimizer capable of finding the global optimum.
 It is clear that fitting a global optimizer is even more unstable than fitting an optimizer with a fixed seed.
 We suspect that this is because, with a fixed seed, the optimizer can only find local optima "near" the seed.
 However, with a global optimizer, we can find the global optimum no matter where it should appear in the search space, so there is more opportunity for the optimum to switch.
 In any case, it seems that in practice, the global optimizer creates highly unstable results.
 This is just as well, because seeding an optimizer with hundreds of seeds is incredibly time-consuming, and results in a significantly less efficient process.

Furthermore, for various covariance functions and data, the sought-after optimum might be in a very "narrow" valley.
 To the point that finding it using a random seed is a rather unlikely event, and so a great number of seeds must be employed to reliably find good optimal paramter estimates.
 This is illustrated in Figure \ref{figure:contrivedperiodgpr}.
 These parameters are extracted by training over the constant and period paramters and fixing the length scale and white noise parameters in Equation \ref{equation:variableperiodcovariance}.
 100 random seeds are chosen log-uniformly on $[10^{-10},10^{10}]$ and the optimizer is run on each of these, with the best result taken in the end.
 Approximately half of the time, a period on the order of tens is found, which is representative of the approximate period of the local data at that point.
 Figure \ref{figure:contrivedperiodgprsmooth} shows a Nadarya-Watson-smoothed version of the curve in Figure \ref{figure:contrivedperiodgpr}.
 Note that the period generally increases toward the middle of the data, and decreases toward the edge, which is reflective of the properties of the underlying data.
 However, the "correct" optimum can be difficult to find, especially for periodic covariance functions where one might reasonably expect a local minimum at factors of the "true" period.
 The result is unstable local parameters over time.

From these observations, we believe that seeding the optimizer with a fixed set of parameters that are near a "normal operating" value to be a good partial solution to the discontinuity problem.
 The proceeding experiments will therefore all employ this option.

Another strategy that can be employed to increase the stability of the results is to reduce the size of the parameter space.
 Specifically, we would a priori expect that an optimization surface over many variables would have more opportunities to play host to superfluous local optima than an optimization surface over fewer variables.
 One way to accomplish this is by `fixing' some of the parameters in the covariance function at convenient values to allow analysis only of parameters of interest.
 Fixing the parameters of the individual models has other side-effects on the model in addition to affecting the stability of the algorithm.
 It is worth noting that a `fixed' parameter essentially becomes a hyperparameter of the algorithm that must be set by some means besides the ordinary training scheme.
 We therefore discuss these effects in the proceeding section

\subsubsection{Setting Hyperparameters} \label{section:hyperparameters}

Similarly to LOESS or kernel density estimation, we must set a kernel bandwidth.
 There has been a great deal of work into bandwidth selection, with a number of reviews covering the subject, for example \cite{turlach1993bandwidth}.
 The effects of bandwidth selection have mostly been considered in relation to local model predictions.
 However, since predictions are generally a function of the parameters, the sundry factors largely translate to the problem at hand.
 Since our datasets contain relatively little data with which to train this hyperparameter, we set it naively using a priori information concerning the nature of our datasets, and do relatively little to explore its effects.

The remaining hyperparameters consist of any fixed parameters in our covariance functions.
 Fixing the parameters in our covariance function may seem to be a strange step from the point of view of attempting to accurately model the data, so we discuss it briefly here.
 We remind the reader that \emph{our purpose here is not to model the data as accurately as possible}.
 Instead, we aim to extract features from the data for an entirely different purpose than interpolation or extrapolation.
 Therefore, the model most suited to interpolation or extrapolation may or may not be the model best suited to our needs.
 Still, any arbitrary model will not do, and we need a ``well-fit" model in some sense.
 It is important to realize that that sense is some combination of the ordinary sense of fitting models (interpolation and extrapolation) but also the extraction of features best suited for whatever the ultimate use of our features will be.
 Such use cases may include change point detection, as in Section \ref{section:accelerometrymethodology}, time series classification, as in Section \ref{section:eegmethodology} or others.

We note that there are 3 "levels" at which we can allow the various parameters to vary.
 At the highest level, allowing it to vary maximally, we could allow a parameter to be trained in the individual local models.
 At this level, a parameter is simply an additional feature extracted from the time series.
 At a middle level, we could fix the parameter during portions of a sequence, or for a single sequence in a group of sequences, but allow it to vary between sequences
 At the lowest level, we could fix the paramter once for the entire sequence or for all sequences in a group using information gleaned from a set of training sequences.
  
The highest level has the ostensible benefit of providing an additional feature that can be used for learning at a later stage.
 It also benefits from the existence of a pre-existing tried-and-true training method, since they would be obtained from the locally-trained GPRs.
 Lastly, it benefits from the ability to show variation in this parameter between different individuals.
 However, this can result in features that are less stable over time, as the optimizer finds various transient local optima.
 A second pitfall is that the various parameters are not independent.
 In other words, we will obtain a different sequence of white noise term parameters depending on whether we fix the constant term and RBF term parameters or not, and will obtain different sequences depending on what levels we fix them at.
 Both of these problems can be witnessed in Figure \ref{figure:allvarscontrivedvariance}.
 It is therefore not clear that the white noise term sequence will benefit from the additional parameter, and in our experience on this and the accelerometry dataset it does not.

The lowest level solves the problems at the highest level associated with learning multiple parameters.
 It may also help alleviate some of the dependence between parameters during GPR training.
 However it suffers from not allowing variation between individual sequences in a group.
 It is also disadvantaged by ignoring potentially valuable information from an additional extracted feature.
 It also requires the creation of a method for choosing an appropriate fixed parameter.
 However, it is not clear that the additional feature is, in fact, useful: recall the previous discussion concerning the distinction between the best parameters for interpolation vs that for activity recognition.
 If we are specifically interested in one particular parameter, and expect relatively little variation in the scale of other parameters between groups, this option may be best.
 In the third set of graphs of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we can see that this plays out.
 In the contrived variance dataset, although there is some change in, e.g., the curvature of the function over time, which may reflect in the learned parameters, the primary feature of change is the noise level.
 By fixing the other parameters at a convenient level, we can focus the method onto changes in one particular variable, control for the dependence between the parameters, and ease the number of discontinuities in the extracted features over time.
 Specifically, the third graph seems to extract the desired signal from the data very well, giving a large value when the noise level is large, and a small value when the noise level is small.

The middle level also solves the problems at the highest level associated with learning two parameters.
 It also has the benefit of allowing a variation in "baseline" readings between individuals.
 Like the lowest level, it may be disadvantaged by losing an additional feature.
 Similarly, it requires the creation of a method for choosing an appropriate fixed parameter.
 Since the parameter is fixed individually for a sequence, the method devised above for choosing a fixed parameter cannot apply if we cannot depend upon having labelled data for every individual.
 One option may be to train a GPR with the parameter allowed to vary on an exemplar segment of data chosen at random from the sequence, and then to subsequently fix the parameter in the local model training to be the value obtained from the exeplar segment.
 This would solve the problem of optimization surface complexity from the highest level.
 However, it would still suffer from having a parameter chosen for the purpose of interpolation rather than activity recognition.
 Furthermore, there is no guarantee that our `exemplar' segment is, in fact, exemplary.
 Since the contrived data do not involve a great deal of variation in the signal, and do not involve signal from multiple individuals, we do not explore this option here.
 Instead, we include discussion related to this possibility with respect to the accelerometry data, we direct the reader to Section \ref{section:accelerometryresults}, and with respect to the eeg data to Section \ref{section:eegmethodology}.












 Indeed, for this dataset, does an "exemplary" segment come from a sequence where a subject was sitting or walking?
 Still, since it not unreasonable to expect that the best parameter for interpolation might yet be a quite good parameter for other purposes, we investigate this method of setting the constant term parameter as well in Section \ref{section:accelerometerresults}.






Note the length scales of the x-axis in Figure \ref{figure:chestaccelerometerZMinutes}.
 Although the signal appears to have a very prominent noise component when viewed at a resolution on the order of minutes, it is significantly less noticeable when we zoom in to see changes at the level of seconds, as seen in Figure \ref{figure:chestaccelerometerZSeconds}.
 This is because there is meaningful small-scale structure to the accelerometer readings.
 However, that small-scale structure is not necessarily useful in distinguishing between various activities.
 In fact, note that the data in Figure \ref{figure:chestaccelerometerZSecondsfixedrbf} is taken during a single activity, suggesting that a good extracted feature for this data should approximate a constant value indicative of the present activity.
 Allowing the optimizer to choose the parameter of the RBF component of our covariance function may therefore not be an optimal method for extracting the noise component.
 Worse, it is possible for the RBF component to, itself, model white noise.
 Specifically, as the length scale of the RBF component goes to 0, the $CN_c RBF_r$ term simply becomes an $WN$ component.
 It is therefore difficult to prevent interactions between these two terms when optimizing our individual local models.
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr}}}
    \caption{An example taken from the chest accelerometry dataset, showing data on the scale of seconds.
        All parameters in the GPR covariance function (Equation \ref{equation:accelerometergpr}) are allowed to vary.
        400 log-uniform seeds are chosen to obtain globally-optimal parameters.
        The optimal RBF length scale is found to be $\approx 0.33s$.
    }
    \label{figure:chestaccelerometerZSeconds}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr_fixed_r}}}
    \caption{The same data from Figure \ref{figure:chestaccelerometerZSeconds}, but with a fixed RBF length scale parameter at $\approx 15s$
        The remaining parameters are allowed to vary.
    }
    \label{figure:chestaccelerometerZSecondsfixedrbf}
\end{figure}



Since we are primarily interested in the noise level term parameter, we further have the constant term parameter to contend with.
 In Section \ref{section:accelerometerresults}, we provide some exploratory investigation into allowing it full freedom to vary along each time series or fixing it to be a particular value for the entire experiment.
 However, as we have noted, there is a strong interaction between the two additive terms in our covariance function.
 Therefore, we have chosen to fix the constant term parameter as well, at a level convenient for change point detection, chosen by manual inspection of the extracted signals.
 Changing the constant parameter has an effect on the sensitivity of the extracted signal, and also on the stability of the extracted signal.
 Low values give a highly unstable signal.
 High values make the feature extraction insensitive to changes in variance, resulting in a "flat-line" for extremely large values.
 An example set of extracted features, where the hyperparameters are chosen to give a good signal by visual inspection, are seen in Figure \ref{figure:accelerometer5}.
 
Indeed, this is exactly the reason why we fixed the \emph{RBF term} parameter.
 Fixing the constant term parameter, however, is not as straightforward as choosing the RBF term paramter.
 Firstly, the more parameters we fix, the more opportunity there is to constrain our model family in such a way that it cannot possibly give a "good" model.
 Secondly, The units of the RBF term parameter are easily interpretable and therefore lend themselves to being fixed according to our a priori conceptions about the data.
 The optimal constant term parameter is related to the overall variance in the signal, but it also depends on the RBF term parameter, and we therefore lack the insight to simply fix it based on our expertise in the subject.
 Although we cannot set it a priori, it seems reasonable that we might simply train this parameter against a training set of accelerometer readings to optimally predict the true labels.
 We investigate such a procedure in Section \ref{section:accelerometerresults}.





First, there are a number of hyperparameters affected execution of the algorithm.
 Recall from Section \ref{section:accelerometrymethodology} that we have an option to fix various parameters of the GPR during local model training.
 If we elect to fix any of the model parameters, the value at which they are fixed can be considered a hyperparameter of the local model feature extraction.
 Lastly, we need to set the bandwidth for our kernel.
 We will investigate here the effect of all of these various hyperparameters on the results of the algorithm, as well as the effects of fixing the various parameters in the local models.
 Instead of providing a full grid over the various hyperparameters, we will take pick and choose what we consider to be representative possibilities that illustrate possible pitfalls and prospects of local model feature transformations with GPR.

One factor compounding the issue of discontinuous local parameters over time is the dimensionality of the parameter space.
 The larger the space, the more opportunity exists for local optima to appear and disappear, and to generally move up, down and around one another over time.
 Thus, if we identify target parameters that we expect to be indicative of particular properties of interest in our time series, we can potentially "fix" the other parameters.
 This potentially has two advantages.
 First, the size of the parameter space is reduced, potentially improving stability of extracted parameters over time.
 Second, problems with interpreting changes in the local parameters due to dependence between the various parameters is reduced, since only a limited set of the parameters are allowed to vary.
 In other words, changes in a non-target parameter do not cause changes in the target parameter, since the non-target parameter is simply not allowed to vary. 
 We direct the reader to Section \ref{section:accelerometrymethodology} for a more thorough discussion of how "fixing" certain parameters is expected to affect the overall procedure.

Figure \ref{figure:contrivedvariancevariousfixedparameters} shows the results of training a local GPR on our contrived dataset while fixing the RBF term and the constant term's parameters (see Equation \ref{equation:variablevariancecovariance}).
 We seed the white noise parameter with a value of $1$ at all points in time, although we note that the particular seed value used does not much affect the results, so long as the seed is fixed.
 
We will here attempt to explain the extracted features in terms of the intuition behind the chosen form of the covariance function.
 This will provide us with a basis for setting the model parameters in future iterations.
 We note that, although these explanations are based largely on the intuitions outlined in \cite{rasmussen2005gaussian}, they are otherwise post hoc.
 Therefore, these explanations should be taken to be hypothetical.
 Although we will not test them directly, we employ them implicitly in constructing later models, and the reader can weigh the evidence for these explanations in part by the procedure's performance on these subsequent experiments.

 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{illustrative_pairs_contrived_variance}}}
    \caption{Variable noise data below in orange.  
    The three sections divided by a horizontal black line are: top - global parameter search, middle - neighboring parameter seed, bottom - fixed parameter seed.
    Within each section, the graphs in blue represent local GPR white noise parameter freatures obtained with fixed $c,r$ at various values.
    From top to bottom, within each section, the $c,r$ pairs are: $(32,8),(64,2),(64,512),(.25,.12)$ and $(.25,2)$}
    \label{figure:contrivedvariancevariousfixedparameters}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{all_vars_contrived_variance}}}
    \caption{Variable noise data below in pink.
        The other graphs represent the various parameters of a locally trained GPR over time.}
    \label{figure:allvarscontrivedvariance}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr}}}
    \caption{Variable period data below in green.
        Extracted gpr parameters are period for the exponential sine squared term in orange, and the constant term value in blue.
        100 seeds are chosen log-uniformly on $[10^{-10}, 10^{10}]$.}
    \label{figure:contrivedperiodgpr}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr_smoothed}}}
    \caption{The same extracted features from Figure \ref{figure:contrivedperiodgpr}, but smoothed by a weighted rolling mean. 
    }
    \label{figure:contrivedperiodgprsmooth}
\end{figure}


 

\subsection{Accelerometry Data} \label{section:accelerometerresults}

%TODO the transformed data are in chest_acc_run019/transformed_data

In this section we discuss the results of the proposed feature extraction algorithm applied to the accelerometry dataset described in Section \ref{section:accelerometrymethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on discovery of change points in time series.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the signals from 2 different individuals.
 A portion of the signal containing the ground truth change points for both sequences can be seen in Figures \ref{figure:accelerometer5} and \ref{figure:accelerometer6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:accelerometrymethodology} is also shown.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_05_y_axis}}}
    \caption{y-axis acceleration from one of the sequences in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_06_z_axis}}}
    \caption{z-axis acceleration from a second sequence in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer6}
\end{figure}

The hyperparameters used in these graphs were chosen from a log-uniform grid search to return the maximum signal upon visual inspection.
 Although we do not include the full results of the grid search, we refer the reader to Section \ref{section:contrivedresults}, and specifically Figure \ref{figure:contrivedvariancevariousfixedparameters} for comparable results on the contrived datasets.

In Section \ref{section:eegmethodology} we describe a process by which an exemplar model may be used to obtain the seed values for local model training.
 However, this process was not found to be effective for the accelerometry dataset. 



\subsubsection{Confirmatory Results}



\subsection{EEG Epilepsy Data} \label{section:eegresults}

In this section we discuss the results of the proposed feature extraction algorithm applied to the eeg dataset described in Section \ref{section:eegmethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on classification of subsequences of the data.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the positive (including ictal onset) subsamples from 2 different individuals.
 The positive samples contain both ictal and non-ictal activity, and were expected to therefore illustrate the differences in the extracted features for these two types of eeg signals.
 A portion of the signal containing the labeled point of ictal onset for both sequences can be seen in Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:eegmethodology} is also shown.
 Some caution is advised in the interpretation of these graphs, since these are our `training' data, and parameters have therefore been specifically selected in such a way as to obtain a `nice' signal.

Some other configurations of hyperparameters were attempted, but did not give pleasing results.
 Notably, in early experiments we attempted to model the data locally using a covariance function with 4 RBF terms.
 Each was set at a length scale corresponding roughly to the various waveforms commonly encountered in brain activity - beta, alpha, theta and delta waves, and the constant value term was allowed to vary locally.
 However, in experiments, the features extracted at the various length scales were highly correlated, resulting in superfluous features.
 Furthermore, the correlation resulted in a situation where the signal represented by one term overlapped sufficiently with the other terms as to frequently cause a deep local optimum at 0 for the other terms.
 It was therefore often the case that one term would dominate, and the resulting signal was highly unstable with the various terms going to 0 at different times.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00019_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from one of the recordings, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00020_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from a second recording, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset6}
\end{figure}

Due to these issues, the single-term configuration was chosen for improved stability at the expense of interpretability.
 We did not experiment with a wide variety of RBF length scales, since the scale characteristic of theta waves gave reasonable results, and we determined that there was insufficient training data to improve upon that scale by manual inspection or otherwise.
 Although the length scale was fixed at a level representative of theta waves, we expect that variations in the constant term over time will still reflect ratios in the various types of brain waves.
 In Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6} it can be seen that sections of the signal with prominent low-frequency components give high values for the extracted feature, and vice-versa.
 In those same figures, it can be seen that the onset of ictal activity generally seems to involve a move from lower-valued LMFT features to higher-valued ones, although perhaps not in a uniform fashion.
 This observation has informed our hypothesis that the performance of DTW will increase when applied to the LMFT features, since it need only discover the relatively simple transition over time from low to high value, rather than an intricate series of ups and downs associated with the raw eeg signals.

\subsubsection{Confirmatory Results}

Having decided upon a covariance function family and a setting for the various hyperparameters in the exploratory analysis, we proceed to extract features from every channel of every sequence.
 We then employ the validation process as described in Section \ref{section:eegmethodology}.

The confusion matrices for the 3 proposed datasets - raw data, LMFT features and the concatenation of the two - are given in Table \ref{table:eegconfusion}.
 It can be seen that 1NN using DTW for classifying sequences of nonictal eeg activity vs the onset of ictal activity using the raw data is ineffective.
 Indeed, the true label and the predicted label are entirely independent.
 Upon inspection, it seems that 17/19 of the true positive and 15/19 of the true negative validation sequences were matched to two of the training sequences.
 Interestingly, although one of those training sequences was true positive and one true negative, there was no correlation to the label of the validation sequences to which they were matched.
 It is not clear what the cause of this strong preference for certain training sequences was, but the lack of correlation reveals that the raw data are not useful for input directly into a classifier.
 
Similarly, when the raw data and the extracted features were concatenated, 34/38 of the validation sequences were matched to two of the training sequences.
 These two sequences were both negative, and were both different from the two popular sequences from the 1NN with DTW on only the raw data.
 We had expected that the combined information of the raw data and the extracted features would be \emph{more} informative for a classification algorithm, but this did not turn out to be the case.

1NN with DTW on only the LMFT features performed better.
 The gains were modest, giving an accuracy, precision and recall of only 0.66, 0.75 and 0.47 respectively. 
 Still, the intention of the experiment was to show that the LMFT extracted features could be useful for a later classification step, and so these results support our hypothesis.
 We remind the reader that there exist opportunities for training over hyperparamters with larger datasets, and also that the proposed algorithm accepts arbitrary model families.
 This suggests that many improvements to the proposed method might still be made, even for this particular task of epilepsy detection.

\begin{table}[h!]
  \begin{center}
    \caption{EEG classification confusion matrices}
    \label{table:eegconfusion}
    \begin{tabular}{llll|ll|ll}
        &   & \multicolumn{6}{c}{\textbf{Predicted}} \\
        &   & \multicolumn{2}{c}{\textbf{Raw Data}} & \multicolumn{2}{c}{\textbf{LMFT}} & \multicolumn{2}{c}{\textbf{Both}} \\
        &   & -    & +    & -    & +    & -    & +    \\
      \multirow{2}{*}{\textbf{True}}
        & - & 14   & 5    & 16   & 3    & 0    & 19   \\
        & + & 14   & 5    & 10   & 9    & 0    & 19
    \end{tabular}
  \end{center}
\end{table}

%TODO We should go and do a post-hoc analysis on why the misclassified ones were misclassified by viewing the extracted features and seeing what the exemplar model was.


==> local_W2V_v_time/results/long_results.tex <==

\section{Results} \label{section:results}

\subsection{Contrived Data} \label{section:contrivedresults}

In this section we investigate a number of practical issues related to obtaining local modeling with Gaussian Processes, including the stability of features over time, hyperparameter selection, and the interpretation of any extracted features.
 We use these initial investigations to inform the setup for later experiments.

\subsubsection{Stability of Extracted Features} \label{section:stability}

At a very basic level, in order for features extracted from a dataset to provide any meaningful insight into the dataset, they should be non-random, and should vary more-or-less continuously with the time-series under consideration.
 By more-or-less continuously, we note that, for example, change point detection algorithms produce non-continuous output in the form of a point-impulse at various locations.
 However, the number of discontinuities in the signal output by a change point detection algorithm are relatively few, and the output features are almost everywhere 0 (indicating no-change).
 On the other hand, features that consist of a very large number of large jump discontinuities are probably not helpful.
 We note this because the algorithm described in Section \ref{section:algorithm} is not mathematically guaranteed to provide stable output.

However, by experiment we show that, by appropriate choice of hyperparameters and other factors, we can encourage a sufficient amount of stability in the extracted features.
 In the remainder of this section, we will explore the underlying mechanisms which might cause instability in the output of the algorithm, and to then propose ways that we might mitigate these issues.

In general, for kernel methods, a smooth kernel gives a smoothly varying optimization surface at each point in time, which results in a smoothly varying optimum over time.
 However, this helpful property does not apply for us, because of the fact that the optimization surface of a GPR is not generally convex.
 Therefore, our algorithm may exhibit discontinuities depending on a variety of factors.
 These include, but are not limited to the choice of seed for the optimizer at each point in time and the number of parameters available to our chosen covariance function.
 Regardless of how we might choose a seed for our optimizer, or various other considerations, however, the output of the algorithm cannot be guaranteed to be continuous.

Before continuing, we would like to examine the continuity claim above that we would have if the optimization surface \emph{were} convex.
 For mathematical simplicity, we only consider here loss functions of the following form, which is a very common form:
%
\begin{equation}
 L(X,\theta,q) = \sum_{x\in X} l(x,\theta)K(x,q)
\end{equation}
%
 Where $X$ is our dataset of size $n$, $l(x,\theta)$ is a bounded loss for a single point $x$, given parameters $\theta$, and $K(x,q)$ is the weight at point $x$ given a query point $q$.
 We are specifically concerned with local weighting schemes, and we will ask what happens to this total loss as the query point changes by a small amount.
 Suppose then, that we have some small quantity in mind, $\delta > 0$ and that $|l(x,\theta)| < M$.
 If $K$ is continuous and symmetric, then we can choose $\epsilon>0$ so that $|K(x,q')-K(x,q)| < \delta/(nM)$ for a given $x$ whenever $|q-q'|<\epsilon$.
 This implies that $|L(X,q',\theta) - L(X,q,\theta)| < \delta$, so that the total loss is also continuous in $q$ at any given $\theta$.
 Our requirement that $l$ be bounded amounts to a bound on $\theta$, but since our dataset $X$ is fixed, this is not an unreasonable requirement for most model families.
 
We would like to see that the optimal parameters $\theta_\text{opt}(q)$ that minimize the total loss at $q$ are also continuous in $q$.
 Choose another $\delta > 0$.

First, observe that for any $\delta > 0$ we can choose an $\gamma > 0$ so that:
$$ \begin{array}{l}L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 This can be acheived by simply setting $\gamma$ so to be the minimum difference $L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q))$ for all $\theta''$ so that $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 To show the contrapositive, choose a $\theta'$ so that $|\theta' - \theta_\text{opt}(q)| > \delta$.
 Choose $\theta''$ to be the point so that $\alpha \theta' + (1-\alpha) \theta_\text{opt}(q) = \theta''$ where $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 Since $L(X,q,\theta)$ is convex in $\theta$ for a given $q$ then:
$$L(X,q,\theta'') < \alpha L(X,q,\theta') + (1-\alpha) L(X,q,\theta_\text{opt}(q))$$
 This gives:
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) \\ > (L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q)))/\alpha \\ > \gamma/\alpha > \gamma \end{array} $$
 
This shows that all of the points $\theta$ that have a ``small" loss are near the current $q$'s optimum.
 We will now combine this fact with $L$'s continuity in $q$ to acheieve the desired result.
 Pick $\gamma > 0$ so that 
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ 
   \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 Further restrict $\gamma$ so that 
$$ \begin{array}{l} L(X,q',\theta') - L(X,q',\theta_\text{opt}(q')) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q')| < \delta/2 \end{array}$$
 Pick $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ \begin{array}{l} 0 < L(X,q',\theta_\text{opt}(q) - L(X,q,\theta_\text{opt}(q) = \\ |L(X,q,\theta_\text{opt}(q)) - L(X,q',\theta_\text{opt}(q))| < \gamma/2 \end{array}$$
 Further restrict $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ L(X,q,\theta_\text{opt}(q')) - L(X,q',\theta_\text{opt}(q')) < \gamma/2$$
 Combining the previous two facts, we have $|q-q'| < \epsilon$ implies 
$$\begin{array}{l} (L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q))) + \\ (L(X,q',\theta_\text{opt}(q) - L(X,q',\theta_\text{opt}(q'))) < \gamma \end{array}$$
 Since $L$ is optimized at $\theta_\text{opt}$, both of these terms are positive, and we have that $L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q)) < \gamma$.
 This implies that $|\theta_\text{opt}(q) - \theta_\text{opt}(q')| < \delta$, which gives the desired result.

In other words, if the optimization surface is convex, then new time series formed by extracted parameters will be continuous.
 If the model family consists of continuous functions, this will further imply a continuous sequence of predictions, which is why LOESS gives continuous curves.
 However, if the optimization surface is \emph{not} convex, then no such continuity is guaranteed.
 Such discontinuities might occur even if the optimization surface is smooth.
 This means that as our time series progresses, the extracted model parameters may experience discontinuities, and these discontinuities are not necessarily related to anything special happening in the data.
 We show this by counterexample.

In Figure \ref{figure:discontinuousoptimaneighboringbeta0}, we show potential loss surfaces over which we intend to optimize a parameter displayed on the $x$ axis.
 Imagine that, as we change $q$, the optimization surface changes at each time step from the function at top to the function at bottom.
 At the top, the loss surface contains a single minimum, which our optimization procedure finds.
 If we seed a gradient descent optimizer with the previous time steps optimum, we will find the points in red.
 Note that this point changes continuously until the local optimum at that point disappears, at which point the optimizer slides to an entirely new local minimum elsewhere.
 The point at which this local minimum disappears will create a discontinuity in the extracted parameters.
 In the case that we use an optimizer that is capable of finding the global minimum at each point, there will be a discontinuity in the optimum at the middle function ($h=1,k=-1$), at which point the two optima have an equal loss.
 In the case that we use a gradient descent optimizer seeded with a constant value, it will experience a discontinuity, but it is not clear at what point that discontinuity will occur.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_neighbor_beta0}}}
    \caption{The family of functions $3x^4-4(k+h)x^3+6khx^2$ for varying values of $h,k$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the previous time-steps optimum.}
    \label{figure:discontinuousoptimaneighboringbeta0}
\end{figure}

Worse, if we seed a gradient descent optimizer with a constant value, the local optima need not disappear in order to experience a discontinuity.
 In Figure \ref{figure:discontinuousoptimaconstantbeta0}, we can see that such a thing might happen.
 Note that this observation also holds for a robust global optimizer that finds the global optimum.
 In the same figure, the two displayed optima have the same loss value, so that a global optimizer might jump between these two values due to small fluctuations.
 Thus, we expect a good global optimizer to actually give \emph{less} stable results than a simple gradient descent optimizer with an appropriate seed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_fixed_beta0}}}
    \caption{The family of functions $(x-h)^4-2(x-h)^2$ for varying values of $h$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the seed at the orage vertical line.}
    \label{figure:discontinuousoptimaconstantbeta0}
\end{figure}

Lastly, we note that, even if a gradient descent optimizer seeded with the previous time-steps optimum does not experience a discontinuity due to the disappearance of the previous time-step's optimum, the local optimum may become very sub-optimal over time.
 Worse, the series of extracted parameters can therefore become `stuck' at a poor local optiumum, and may remain there for the entire time series.

So, we see that when the optimization surface is not guaranteed to be convex, the extracted features cannot be guaranteed to be continuous.
 However, the strategy by which we seed the optimizer can have an effect on the stability of the results.
 We consider here, empirically, the 3 optimizer strategies discussed above: constant seed, seed with neighboring interval optimum value, and global optimization.

All of these options can be seen in practice in Figure \ref{figure:contrivedvariancevariousfixedparameters}, displaying results from the various seed strategies, and also for various selections for fixing covariance function hyperparameters, which we discuss later in this section.
 In each of the graphs in Figure \ref{figure:contrivedvariancevariousfixedparameters}, the constant term and RBF term parameters are fixed to various values, and the optimizer for the remaining white noise term $w$ is seeded according to various strategies.

In the third set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we simply seed the the optimizer with a starting value that is equal to the fixed constant term value used for that set of features. 
 This seed is employed at every point in time.
 In the 1st and 5th graph down, we can see that some choices of hyperparameters can result in an unstable set of features.
 However, in the 2nd, 3rd and 4th graphs, we can see that a good choice of hyperparameters can result in a more stable set of features.

In the second set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters} we seed the optimizer with the optimum found at the previous point in time.
 We can see in 1st and 3rd graphs that, although the extracted parameters seem to pick up on the change in white noise level, they do not readily return to `normal' levels after the period of altered noise.
 This suggests that they have become `stuck' at a suboptimal local minimum.
 Worse, the 1st, 3rd and 5th graphs suggest that the strategy of seeding the optimizer with a neighboring query point's optimal parameters is not as helpful in encouraging stability as we might have hoped.

In the top set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we seed the optimizer with both the previous time step's optimal parameters and also the exemplar period.
 If the optimum found by seeding with the exemplar parameters has a higher marginal likelihood than at the optimum found by seeding with the neighboring optimum, we fit a GPR with hundreds of seeds spread log-uniformly throughout the parameter space.
 This emulates fitting an optimizer capable of finding the global optimum.
 It is clear that fitting a global optimizer is even more unstable than fitting an optimizer with a fixed seed.
 We suspect that this is because, with a fixed seed, the optimizer can only find local optima "near" the seed.
 However, with a global optimizer, we can find the global optimum no matter where it should appear in the search space, so there is more opportunity for the optimum to switch.
 In any case, it seems that in practice, the global optimizer creates highly unstable results.
 This is just as well, because seeding an optimizer with hundreds of seeds is incredibly time-consuming, and results in a significantly less efficient process.

Furthermore, for various covariance functions and data, the sought-after optimum might be in a very "narrow" valley.
 To the point that finding it using a random seed is a rather unlikely event, and so a great number of seeds must be employed to reliably find good optimal paramter estimates.
 This is illustrated in Figure \ref{figure:contrivedperiodgpr}.
 These parameters are extracted by training over the constant and period paramters and fixing the length scale and white noise parameters in Equation \ref{equation:variableperiodcovariance}.
 100 random seeds are chosen log-uniformly on $[10^{-10},10^{10}]$ and the optimizer is run on each of these, with the best result taken in the end.
 Approximately half of the time, a period on the order of tens is found, which is representative of the approximate period of the local data at that point.
 Figure \ref{figure:contrivedperiodgprsmooth} shows a Nadarya-Watson-smoothed version of the curve in Figure \ref{figure:contrivedperiodgpr}.
 Note that the period generally increases toward the middle of the data, and decreases toward the edge, which is reflective of the properties of the underlying data.
 However, the "correct" optimum can be difficult to find, especially for periodic covariance functions where one might reasonably expect a local minimum at factors of the "true" period.
 The result is unstable local parameters over time.

From these observations, we believe that seeding the optimizer with a fixed set of parameters that are near a "normal operating" value to be a good partial solution to the discontinuity problem.
 The proceeding experiments will therefore all employ this option.

Another strategy that can be employed to increase the stability of the results is to reduce the size of the parameter space.
 Specifically, we would a priori expect that an optimization surface over many variables would have more opportunities to play host to superfluous local optima than an optimization surface over fewer variables.
 One way to accomplish this is by `fixing' some of the parameters in the covariance function at convenient values to allow analysis only of parameters of interest.
 Fixing the parameters of the individual models has other side-effects on the model in addition to affecting the stability of the algorithm.
 It is worth noting that a `fixed' parameter essentially becomes a hyperparameter of the algorithm that must be set by some means besides the ordinary training scheme.
 We therefore discuss these effects in the proceeding section

\subsubsection{Setting Hyperparameters} \label{section:hyperparameters}

Similarly to LOESS or kernel density estimation, we must set a kernel bandwidth.
 There has been a great deal of work into bandwidth selection, with a number of reviews covering the subject, for example \cite{turlach1993bandwidth}.
 The effects of bandwidth selection have mostly been considered in relation to local model predictions.
 However, since predictions are generally a function of the parameters, the sundry factors largely translate to the problem at hand.
 Since our datasets contain relatively little data with which to train this hyperparameter, we set it naively using a priori information concerning the nature of our datasets, and do relatively little to explore its effects.

The remaining hyperparameters consist of any fixed parameters in our covariance functions.
 Fixing the parameters in our covariance function may seem to be a strange step from the point of view of attempting to accurately model the data, so we discuss it briefly here.
 We remind the reader that \emph{our purpose here is not to model the data as accurately as possible}.
 Instead, we aim to extract features from the data for an entirely different purpose than interpolation or extrapolation.
 Therefore, the model most suited to interpolation or extrapolation may or may not be the model best suited to our needs.
 Still, any arbitrary model will not do, and we need a ``well-fit" model in some sense.
 It is important to realize that that sense is some combination of the ordinary sense of fitting models (interpolation and extrapolation) but also the extraction of features best suited for whatever the ultimate use of our features will be.
 Such use cases may include change point detection, as in Section \ref{section:accelerometrymethodology}, time series classification, as in Section \ref{section:eegmethodology} or others.

We note that there are 3 "levels" at which we can allow the various parameters to vary.
 At the highest level, allowing it to vary maximally, we could allow a parameter to be trained in the individual local models.
 At this level, a parameter is simply an additional feature extracted from the time series.
 At a middle level, we could fix the parameter during portions of a sequence, or for a single sequence in a group of sequences, but allow it to vary between sequences
 At the lowest level, we could fix the paramter once for the entire sequence or for all sequences in a group using information gleaned from a set of training sequences.
  
The highest level has the ostensible benefit of providing an additional feature that can be used for learning at a later stage.
 It also benefits from the existence of a pre-existing tried-and-true training method, since they would be obtained from the locally-trained GPRs.
 Lastly, it benefits from the ability to show variation in this parameter between different individuals.
 However, this can result in features that are less stable over time, as the optimizer finds various transient local optima.
 A second pitfall is that the various parameters are not independent.
 In other words, we will obtain a different sequence of white noise term parameters depending on whether we fix the constant term and RBF term parameters or not, and will obtain different sequences depending on what levels we fix them at.
 Both of these problems can be witnessed in Figure \ref{figure:allvarscontrivedvariance}.
 It is therefore not clear that the white noise term sequence will benefit from the additional parameter, and in our experience on this and the accelerometry dataset it does not.

The lowest level solves the problems at the highest level associated with learning multiple parameters.
 It may also help alleviate some of the dependence between parameters during GPR training.
 However it suffers from not allowing variation between individual sequences in a group.
 It is also disadvantaged by ignoring potentially valuable information from an additional extracted feature.
 It also requires the creation of a method for choosing an appropriate fixed parameter.
 However, it is not clear that the additional feature is, in fact, useful: recall the previous discussion concerning the distinction between the best parameters for interpolation vs that for activity recognition.
 If we are specifically interested in one particular parameter, and expect relatively little variation in the scale of other parameters between groups, this option may be best.
 In the third set of graphs of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we can see that this plays out.
 In the contrived variance dataset, although there is some change in, e.g., the curvature of the function over time, which may reflect in the learned parameters, the primary feature of change is the noise level.
 By fixing the other parameters at a convenient level, we can focus the method onto changes in one particular variable, control for the dependence between the parameters, and ease the number of discontinuities in the extracted features over time.
 Specifically, the third graph seems to extract the desired signal from the data very well, giving a large value when the noise level is large, and a small value when the noise level is small.

The middle level also solves the problems at the highest level associated with learning two parameters.
 It also has the benefit of allowing a variation in "baseline" readings between individuals.
 Like the lowest level, it may be disadvantaged by losing an additional feature.
 Similarly, it requires the creation of a method for choosing an appropriate fixed parameter.
 Since the parameter is fixed individually for a sequence, the method devised above for choosing a fixed parameter cannot apply if we cannot depend upon having labelled data for every individual.
 One option may be to train a GPR with the parameter allowed to vary on an exemplar segment of data chosen at random from the sequence, and then to subsequently fix the parameter in the local model training to be the value obtained from the exeplar segment.
 This would solve the problem of optimization surface complexity from the highest level.
 However, it would still suffer from having a parameter chosen for the purpose of interpolation rather than activity recognition.
 Furthermore, there is no guarantee that our `exemplar' segment is, in fact, exemplary.
 Since the contrived data do not involve a great deal of variation in the signal, and do not involve signal from multiple individuals, we do not explore this option here.
 Instead, we include discussion related to this possibility with respect to the accelerometry data, we direct the reader to Section \ref{section:accelerometryresults}, and with respect to the eeg data to Section \ref{section:eegmethodology}.












 Indeed, for this dataset, does an "exemplary" segment come from a sequence where a subject was sitting or walking?
 Still, since it not unreasonable to expect that the best parameter for interpolation might yet be a quite good parameter for other purposes, we investigate this method of setting the constant term parameter as well in Section \ref{section:accelerometerresults}.






Note the length scales of the x-axis in Figure \ref{figure:chestaccelerometerZMinutes}.
 Although the signal appears to have a very prominent noise component when viewed at a resolution on the order of minutes, it is significantly less noticeable when we zoom in to see changes at the level of seconds, as seen in Figure \ref{figure:chestaccelerometerZSeconds}.
 This is because there is meaningful small-scale structure to the accelerometer readings.
 However, that small-scale structure is not necessarily useful in distinguishing between various activities.
 In fact, note that the data in Figure \ref{figure:chestaccelerometerZSecondsfixedrbf} is taken during a single activity, suggesting that a good extracted feature for this data should approximate a constant value indicative of the present activity.
 Allowing the optimizer to choose the parameter of the RBF component of our covariance function may therefore not be an optimal method for extracting the noise component.
 Worse, it is possible for the RBF component to, itself, model white noise.
 Specifically, as the length scale of the RBF component goes to 0, the $CN_c RBF_r$ term simply becomes an $WN$ component.
 It is therefore difficult to prevent interactions between these two terms when optimizing our individual local models.
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr}}}
    \caption{An example taken from the chest accelerometry dataset, showing data on the scale of seconds.
        All parameters in the GPR covariance function (Equation \ref{equation:accelerometergpr}) are allowed to vary.
        400 log-uniform seeds are chosen to obtain globally-optimal parameters.
        The optimal RBF length scale is found to be $\approx 0.33s$.
    }
    \label{figure:chestaccelerometerZSeconds}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr_fixed_r}}}
    \caption{The same data from Figure \ref{figure:chestaccelerometerZSeconds}, but with a fixed RBF length scale parameter at $\approx 15s$
        The remaining parameters are allowed to vary.
    }
    \label{figure:chestaccelerometerZSecondsfixedrbf}
\end{figure}



Since we are primarily interested in the noise level term parameter, we further have the constant term parameter to contend with.
 In Section \ref{section:accelerometerresults}, we provide some exploratory investigation into allowing it full freedom to vary along each time series or fixing it to be a particular value for the entire experiment.
 However, as we have noted, there is a strong interaction between the two additive terms in our covariance function.
 Therefore, we have chosen to fix the constant term parameter as well, at a level convenient for change point detection, chosen by manual inspection of the extracted signals.
 Changing the constant parameter has an effect on the sensitivity of the extracted signal, and also on the stability of the extracted signal.
 Low values give a highly unstable signal.
 High values make the feature extraction insensitive to changes in variance, resulting in a "flat-line" for extremely large values.
 An example set of extracted features, where the hyperparameters are chosen to give a good signal by visual inspection, are seen in Figure \ref{figure:accelerometer5}.
 
Indeed, this is exactly the reason why we fixed the \emph{RBF term} parameter.
 Fixing the constant term parameter, however, is not as straightforward as choosing the RBF term paramter.
 Firstly, the more parameters we fix, the more opportunity there is to constrain our model family in such a way that it cannot possibly give a "good" model.
 Secondly, The units of the RBF term parameter are easily interpretable and therefore lend themselves to being fixed according to our a priori conceptions about the data.
 The optimal constant term parameter is related to the overall variance in the signal, but it also depends on the RBF term parameter, and we therefore lack the insight to simply fix it based on our expertise in the subject.
 Although we cannot set it a priori, it seems reasonable that we might simply train this parameter against a training set of accelerometer readings to optimally predict the true labels.
 We investigate such a procedure in Section \ref{section:accelerometerresults}.





First, there are a number of hyperparameters affected execution of the algorithm.
 Recall from Section \ref{section:accelerometrymethodology} that we have an option to fix various parameters of the GPR during local model training.
 If we elect to fix any of the model parameters, the value at which they are fixed can be considered a hyperparameter of the local model feature extraction.
 Lastly, we need to set the bandwidth for our kernel.
 We will investigate here the effect of all of these various hyperparameters on the results of the algorithm, as well as the effects of fixing the various parameters in the local models.
 Instead of providing a full grid over the various hyperparameters, we will take pick and choose what we consider to be representative possibilities that illustrate possible pitfalls and prospects of local model feature transformations with GPR.

One factor compounding the issue of discontinuous local parameters over time is the dimensionality of the parameter space.
 The larger the space, the more opportunity exists for local optima to appear and disappear, and to generally move up, down and around one another over time.
 Thus, if we identify target parameters that we expect to be indicative of particular properties of interest in our time series, we can potentially "fix" the other parameters.
 This potentially has two advantages.
 First, the size of the parameter space is reduced, potentially improving stability of extracted parameters over time.
 Second, problems with interpreting changes in the local parameters due to dependence between the various parameters is reduced, since only a limited set of the parameters are allowed to vary.
 In other words, changes in a non-target parameter do not cause changes in the target parameter, since the non-target parameter is simply not allowed to vary. 
 We direct the reader to Section \ref{section:accelerometrymethodology} for a more thorough discussion of how "fixing" certain parameters is expected to affect the overall procedure.

Figure \ref{figure:contrivedvariancevariousfixedparameters} shows the results of training a local GPR on our contrived dataset while fixing the RBF term and the constant term's parameters (see Equation \ref{equation:variablevariancecovariance}).
 We seed the white noise parameter with a value of $1$ at all points in time, although we note that the particular seed value used does not much affect the results, so long as the seed is fixed.
 
We will here attempt to explain the extracted features in terms of the intuition behind the chosen form of the covariance function.
 This will provide us with a basis for setting the model parameters in future iterations.
 We note that, although these explanations are based largely on the intuitions outlined in \cite{rasmussen2005gaussian}, they are otherwise post hoc.
 Therefore, these explanations should be taken to be hypothetical.
 Although we will not test them directly, we employ them implicitly in constructing later models, and the reader can weigh the evidence for these explanations in part by the procedure's performance on these subsequent experiments.

 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{illustrative_pairs_contrived_variance}}}
    \caption{Variable noise data below in orange.  
    The three sections divided by a horizontal black line are: top - global parameter search, middle - neighboring parameter seed, bottom - fixed parameter seed.
    Within each section, the graphs in blue represent local GPR white noise parameter freatures obtained with fixed $c,r$ at various values.
    From top to bottom, within each section, the $c,r$ pairs are: $(32,8),(64,2),(64,512),(.25,.12)$ and $(.25,2)$}
    \label{figure:contrivedvariancevariousfixedparameters}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{all_vars_contrived_variance}}}
    \caption{Variable noise data below in pink.
        The other graphs represent the various parameters of a locally trained GPR over time.}
    \label{figure:allvarscontrivedvariance}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr}}}
    \caption{Variable period data below in green.
        Extracted gpr parameters are period for the exponential sine squared term in orange, and the constant term value in blue.
        100 seeds are chosen log-uniformly on $[10^{-10}, 10^{10}]$.}
    \label{figure:contrivedperiodgpr}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr_smoothed}}}
    \caption{The same extracted features from Figure \ref{figure:contrivedperiodgpr}, but smoothed by a weighted rolling mean. 
    }
    \label{figure:contrivedperiodgprsmooth}
\end{figure}


 

\subsection{Accelerometry Data} \label{section:accelerometerresults}

%TODO the transformed data are in chest_acc_run019/transformed_data

In this section we discuss the results of the proposed feature extraction algorithm applied to the accelerometry dataset described in Section \ref{section:accelerometrymethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on discovery of change points in time series.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the signals from 2 different individuals.
 A portion of the signal containing the ground truth change points for both sequences can be seen in Figures \ref{figure:accelerometer5} and \ref{figure:accelerometer6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:accelerometrymethodology} is also shown.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_05_y_axis}}}
    \caption{y-axis acceleration from one of the sequences in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_06_z_axis}}}
    \caption{z-axis acceleration from a second sequence in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer6}
\end{figure}

The hyperparameters used in these graphs were chosen from a log-uniform grid search to return the maximum signal upon visual inspection.
 Although we do not include the full results of the grid search, we refer the reader to Section \ref{section:contrivedresults}, and specifically Figure \ref{figure:contrivedvariancevariousfixedparameters} for comparable results on the contrived datasets.

In Section \ref{section:eegmethodology} we describe a process by which an exemplar model may be used to obtain the seed values for local model training.
 However, this process was not found to be effective for the accelerometry dataset. 



\subsubsection{Confirmatory Results}



\subsection{EEG Epilepsy Data} \label{section:eegresults}

In this section we discuss the results of the proposed feature extraction algorithm applied to the eeg dataset described in Section \ref{section:eegmethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on classification of subsequences of the data.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the positive (including ictal onset) subsamples from 2 different individuals.
 The positive samples contain both ictal and non-ictal activity, and were expected to therefore illustrate the differences in the extracted features for these two types of eeg signals.
 A portion of the signal containing the labeled point of ictal onset for both sequences can be seen in Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:eegmethodology} is also shown.
 Some caution is advised in the interpretation of these graphs, since these are our `training' data, and parameters have therefore been specifically selected in such a way as to obtain a `nice' signal.

Some other configurations of hyperparameters were attempted, but did not give pleasing results.
 Notably, in early experiments we attempted to model the data locally using a covariance function with 4 RBF terms.
 Each was set at a length scale corresponding roughly to the various waveforms commonly encountered in brain activity - beta, alpha, theta and delta waves, and the constant value term was allowed to vary locally.
 However, in experiments, the features extracted at the various length scales were highly correlated, resulting in superfluous features.
 Furthermore, the correlation resulted in a situation where the signal represented by one term overlapped sufficiently with the other terms as to frequently cause a deep local optimum at 0 for the other terms.
 It was therefore often the case that one term would dominate, and the resulting signal was highly unstable with the various terms going to 0 at different times.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00019_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from one of the recordings, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00020_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from a second recording, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset6}
\end{figure}

Due to these issues, the single-term configuration was chosen for improved stability at the expense of interpretability.
 We did not experiment with a wide variety of RBF length scales, since the scale characteristic of theta waves gave reasonable results, and we determined that there was insufficient training data to improve upon that scale by manual inspection or otherwise.
 Although the length scale was fixed at a level representative of theta waves, we expect that variations in the constant term over time will still reflect ratios in the various types of brain waves.
 In Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6} it can be seen that sections of the signal with prominent low-frequency components give high values for the extracted feature, and vice-versa.
 In those same figures, it can be seen that the onset of ictal activity generally seems to involve a move from lower-valued LMFT features to higher-valued ones, although perhaps not in a uniform fashion.
 This observation has informed our hypothesis that the performance of DTW will increase when applied to the LMFT features, since it need only discover the relatively simple transition over time from low to high value, rather than an intricate series of ups and downs associated with the raw eeg signals.

\subsubsection{Confirmatory Results}

Having decided upon a covariance function family and a setting for the various hyperparameters in the exploratory analysis, we proceed to extract features from every channel of every sequence.
 We then employ the validation process as described in Section \ref{section:eegmethodology}.

The confusion matrices for the 3 proposed datasets - raw data, LMFT features and the concatenation of the two - are given in Table \ref{table:eegconfusion}.
 It can be seen that 1NN using DTW for classifying sequences of nonictal eeg activity vs the onset of ictal activity using the raw data is ineffective.
 Indeed, the true label and the predicted label are entirely independent.
 Upon inspection, it seems that 17/19 of the true positive and 15/19 of the true negative validation sequences were matched to two of the training sequences.
 Interestingly, although one of those training sequences was true positive and one true negative, there was no correlation to the label of the validation sequences to which they were matched.
 It is not clear what the cause of this strong preference for certain training sequences was, but the lack of correlation reveals that the raw data are not useful for input directly into a classifier.
 
Similarly, when the raw data and the extracted features were concatenated, 34/38 of the validation sequences were matched to two of the training sequences.
 These two sequences were both negative, and were both different from the two popular sequences from the 1NN with DTW on only the raw data.
 We had expected that the combined information of the raw data and the extracted features would be \emph{more} informative for a classification algorithm, but this did not turn out to be the case.

1NN with DTW on only the LMFT features performed better.
 The gains were modest, giving an accuracy, precision and recall of only 0.66, 0.75 and 0.47 respectively. 
 Still, the intention of the experiment was to show that the LMFT extracted features could be useful for a later classification step, and so these results support our hypothesis.
 We remind the reader that there exist opportunities for training over hyperparamters with larger datasets, and also that the proposed algorithm accepts arbitrary model families.
 This suggests that many improvements to the proposed method might still be made, even for this particular task of epilepsy detection.

\begin{table}[h!]
  \begin{center}
    \caption{EEG classification confusion matrices}
    \label{table:eegconfusion}
    \begin{tabular}{llll|ll|ll}
        &   & \multicolumn{6}{c}{\textbf{Predicted}} \\
        &   & \multicolumn{2}{c}{\textbf{Raw Data}} & \multicolumn{2}{c}{\textbf{LMFT}} & \multicolumn{2}{c}{\textbf{Both}} \\
        &   & -    & +    & -    & +    & -    & +    \\
      \multirow{2}{*}{\textbf{True}}
        & - & 14   & 5    & 16   & 3    & 0    & 19   \\
        & + & 14   & 5    & 10   & 9    & 0    & 19
    \end{tabular}
  \end{center}
\end{table}

%TODO We should go and do a post-hoc analysis on why the misclassified ones were misclassified by viewing the extracted features and seeing what the exemplar model was.


==> local_gpr/methodology/long_methodology.tex <==

\section{Methodology} \label{section:methodology}

\subsection{Algorithm} \label{section:algorithm}

We propose a method of automatic feature extraction that maps the original data to new vectors representing local relationships between data points.
 This method, based in part on the algorithm in \cite{bay2004framework}, consists of training a model at each point in a domain where data are weighted in such a way as to obtain a `local' model.
 Various properties of these local models, such as the model parameters, can then be extracted as features for further analysis.
 
We employ the concept of kernel methods to localize our model training algorithm.
 This involves weighting data that are `near' a query point $q$ to obtain a local model at the point $q$ using a kernel $K$.

 Common choices for $K$ include a uniform kernel, which, for time-series, is equivalent to a Parzen window:
%
 \begin{equation}
    U_h(x,x') =
        \begin{cases}
            1 & ||x-x'||<h \\
            0 & \text{else} \\
        \end{cases}
\end{equation}
%
 And also a tricube kernel, which transitions the weights of distant points smoothly to 0:
%
 \begin{equation} \label{equation:tricube}
    T_h(x,x') = (1-||x-x'||^3)^3
 \end{equation}
%
 The general idea of learning a local model using a kernel-weighting scheme can be found in expositions of the LOESS procedure \cite{cleveland1979robust}.
 
We then extract the parameters of the local model to obtain the state of the process at the point $q$.
 Our analyses may involve preprocessing of data and further processing to obtain specific results, but the primary contribution of this paper is the above described feature extraction method.

More formally, and generally, consider a dataset $X$ on some domain $D$, and a model family $F$ parameterized by $\theta$.
 Suppose that $A$ is an algorithm for training a model that takes in $X$ and returns $f \in F$, and that $A$ accepts a scheme for weighting the contributions of the individual datapoints.
 Points $x\in X$ are weighted against the query point $q$, usually as some function of their distance to $q$, as $K(x,q)$.
 We denote the weighted training procedure at query point $q$, weighted using kernel $K$ as $A_{K,q}$.
 If $P$ is some model postprocessing algorithm, $P: F\rightarrow {\rm I\!R^k}$, then we can compose $A$ and $P$ on the dataset $X$ to obtain a feature transformation from the original variables to a new space that encodes local structure of the data.
 We term this transformation a `Local Model Feature Transformation' (LMFT):
%
\begin{equation} \label{equation:lmft}
  LMFT(q) = P(A_{K,q}(X))
\end{equation}
%
 This broad class of functions includes local model predictions, local model parameters and other summarizing statistics for individual local models.
 The manner of local structure that is encoded depends on the specific choice of $F$, $A$, $K$ and $P$, but primarily on $F$ and $P$.
 
For the purposes of this paper will will be studying the family of functions $F$ defined by Gaussian Process Regression (GPR) using a covariance function that is context-specific (see Section \ref{section:gpr}).
 We weight our GPR algorithm according to a weighting scheme similar to that described in \cite{hong2017weighted}.
 This weighting scheme, the intuition behind it and some basic theoretical results are included in the Appendix.
 Except for the addition of a weighting scheme, we employ the `ordinary' training procedure ($A$) of optimizing the marginal likelihood over available model parameters \cite{rasmussen2005gaussian}.
 
We will employ the tricube kernel for $K$ (Equation \ref{equation:tricube}) throughout our experiments, since it is smooth and also since it has a finite support which is more computationally efficient.
 The tricube kernel requires one free parameter, the bandwidth $h$, which essentially sets the width of the window, and must be appropriately chosen given the context.
 
Lastly, our postprocessing procedure $P$ will consist of simply extracting the parameters of the locally-trained models.
 Since these parameters are real, we obtain a new time-series in the space of model parameters.
 In the proceeding sections, and especially Section \ref{section:contrivedresults}, we provide an intuition into this new time-series and also demonstrate its potential real-world applications.

\subsection{Experiments}

In this section, we describe the datasets used, and the methods employed to provide evidence for the utility of the algorithm described in \ref{section:algorithm}.
 Since the intent of the given procedure is to provide a generic framework for extracting signals from data, we have attempted to provide a variety of contrived and real world datasets to illustrate the algorithm's flexibility.

\subsubsection{Contrived Data} \label{section:contriveddata}

We have contrived datasets that reflect both changes in levels of white noise and also in periodicity. 
 These two datasets can be seen in Figures \ref{figure:contrivedvariancevariousfixedparameters} and \ref{figure:contrivedperiodgpr}, respectively.
 We provide these to illustrate the general idea, and to provide evidence enough to warrant exploration on real data.
 We further attempt to provide here justifications for some of the decisions made in later experiments regarding choice of various hyperparameters, and other design decisions.
 Thus, we will not perform any validation in the ordinary sense, and will instead merely provide visualizations of cherry-picked results intended to provide the reader with a `feel' for the algorithm.
 
We investigate two contrived datasets to explore the ability of the method to model changes in different properties of a time series.
 Our first contrived dataset consists of a simple sine curve $y = 10 \sin(\frac{2\pi}{50}x)$, with added Gaussian noise.
 The noise has mean 0, and variance 1 during the majority of the sequence, but has variance 5 between points 450 and 550.
 This dataset is designed to illustrate the algorithm's handling of data with varying white noise levels.

The second dataset consists of a sine curve with period dependent on $x$: $y = 10 \sin\frac{2\pi x^2}{20000}$ on $[-500,500]$ with added noise $\sim N(0,1)$ along the entire domain.
 This dataset is designed to illustrate the algorithm's handling of data with varying period.

We note that these are not the extent of parameters available to a Gaussian Process Regression, and certainly do not cover the extent of parameters available when wider classes of model families are taken under consideration.
 However, investigating the changes in multiple different parameters shows that the algorithm can have a range of uses with minimal change to the general structure of the process.

Analysis of the first datset will employ a covariance function of the form:
%
\begin{equation} \label{equation:variablevariancecovariance}
 C = CN_c RBF_r + WN_w
\end{equation}
%
 Analysis of the second dataset will employ a covariance function of the form:
%
\begin{equation} \label{equation:variableperiodcovariance}
 C = CN_c SS_{p,l} + WN_w
\end{equation}
%
 
We employ a tricube kernel to locally weight our data during training of individual models, with a bandwidth of 120.
 We have chosen the value 120 a priori, since this results in a `window' of size $240$ and the length of the section we wish to detect is of length $100$ in the variable noise dataset.
 We have not attempted to evaluate the effect of bandwidth, but the reader may wish to keep in mind that, in general, a higher bandwidth tends to produce smoother results, as is typical with kernel methods \cite{turlach1993bandwidth}.

\subsubsection{Accelerometry Data} \label{section:accelerometrymethodology}

In order to demonstrate that the algorithm is useful for real-world applications, we further provide analyses of a set of uncalibrated accelerometer readings previously used for activity classification \cite{casale2011human}.
 An example of one axis of one set of observations from this dataset is given in Figure \ref{figure:accelerometer5}.
 We will employ this same dataset, but we will only try to detect when there has been a change in activity.
 This is an important sub-problem in the task of classifying individual activities, and is a simplification of the problem suitable for initial explorations of the proposed algorithm.
 It is easy to see from Figure \ref{figure:accelerometer5} that an important feature for detecting a change in activity is the amount of noise in the signal.
 This makes intuitive sense as well: the amount of `bounce' picked up by the accelerometer will be significantly different depending on whether one is sitting at a computer or running up a flight of stairs.

Unfortunately, from the figure, we can see that the accelerometer doesn't seem to hold its zero very well, and there may therefore be longer-term trends in the accelerometer values.
 It also seems as though there may be sudden shifts in the mean.
 Although these sudden mean shifts occasionally align with a change in activity, it is just as frequent that they occur when there is no change in activity.
 Possibly this is due to an individual performing a sudden action while sitting down, such as turning or leaning back.
 Since there is no label for such things, it is only clear that such shifts are not necessarily indicative of a change in activity.
 We hypothesize that it would be possible to extract these changes in noise level while simultaneously accounting for the longer-term trends and shifts in mean with a local GPR with a covariance function of the form:

\begin{equation} \label{equation:accelerometergpr}
    C = CN_c RBF_r + WN_w %TODO: we need to pick names for the parameters
\end{equation}
%
The RBF term will account for the observed trends and shifts to the mean.
By monitoring the changes in the learned parameter for the white noise component, which is obtained conditional upon the RBF term, we hope to extract a signal that clearly indicates when there has been a change in activity.


We impose restrictions to force the RBF term to ignore very small scale changes, while still modeling the long-term changes in accelerometer calibration mentioned above.
 We acheive this by fixing the length scale parameter of the RBF component to be relatively large, and also by fixing the constant term parameter to reflect the scale of the data.
 These values are chosen from a log2-uniform grid search over $r$ and $c$.
 Since the ultimate goal of the procedure is to detect change points, we choose $r$ and $c$ to optimize the detection of change points.
 We set aside 7 sequences for training these algorithm hyperparameters, and leave the remaining 8 for validation.
 Some exploratory analysis lending evidence to our decision to fix these values rather than allowing them to vary in the model is discussed in Section \ref{section:accelerometerresults}.
 Fixing various parameters in our local models has further benefits which we describe in Section \ref{section:contrivedresults}.
 
The local models are weighted by a tricube kernel with a bandwidth that was also chosen via grid search over the training data.
 Larger bandwidths have the effect of ``smoothing out" point anomalies at the expense of potentially losing short-duration changes.

For each combination of hyperparameters defining our model family, we propose to extract local GPR features from each channel of an accelerometer recording, resulting in a $N_t\times N_c \times N_f$ tensor, where $N_t$ is the recording length, $N_c$ is the number of channels (3), and $N_f$ is the number of features extracted from each channel.
 We then flatten the last two axes to re-obtain a time-series of vectors allowing traditional analysis, resulting in a transformed dataset of shape $N_t\times N_cN_f$.
 If we constrain the problem so that the white noise level is our only free parameter, this results in a new time series with 3 channels, each representing the local noise-level of the accelerometer readings in each axis.
 When the constant term parameter is also free, we obtain 6 channels.

For change point detection, we employ the PELT detector \cite{killick2012optimal} as implemented in \cite{truong2018ruptures} using the NMCD cost function described in \cite{zou2014nonparametric}.
 PELT takes a single hyperparameter that penalizes greater numbers of change points.
 We choose this hyperparameter via a grid search over possible penalty parameters on the training set.
 All of the parameters over which we optimize are chosen to maximize the overall F1-score.
 We employ the F1-score since it is mentioned in the list of possible evaluation metrics in \cite{truong2018selective}, since we will report validation results later in terms of precision and recall, and since accuracy is ill-defined for change-point detection.

Validation is performed on three separate sets of features: the LMFT-extracted features, the original raw data, and the concatenation of the two.
 We then compare the confusion matrices of these three possibilities in order to validate the utility of the extracted features.

Upon inspection, the labels in the dataset provided on the UCI machine learning repo do not seem to align perfectly with the signal in the time series.
 An example is shown in Figure \ref{figure:misalignedlabels}.
 The original authors were unreachable for comment.
 Since the dataset is relatively small, we have gone through and manually aligned the ground-truth labels by applying a constant shift to the entire label sequence.
 This was performed as a preprocessing step, before any change-point-detection was applied.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_misalignment}}}
    \caption[Raw accelerometry readings]{Raw accelerometry readings.  
        Obtained from one of the sequences in the UCI accelerometry dataset.
        Vertical lines are ground-truth labels indicating activity change.}
    \label{figure:misalignedlabels}
\end{figure}

Still, the alignment of the ground-truth labels is not perfect - performed, as it were, upon the data zoomed at the order of minutes.
 We have therefore chosen to use a rather liberal threshhold for marking a `true positive' of 10s.
 Since the duration of various activities tends to be on the order of minutes, we think that this is not totally unreasonable.
 Furthermore, we employ the alignment and this same threshold for both the LMFT sequences and the raw data sequences, so that these steps are expected to add variance to the interpretation of the results, rather than bias. 

To summarize, the preprocessing consists solely of aligning what seem to be misaligned labels.
The training process is as follows:
%
\begin{enumerate}
 \item For various parameters of the LMFT procedure, apply local GPR to all channels of the training sequences, obtaining a new sequence of LMFT-features.
 \item For various values of the `penalty' parameter, apply PELT/NMCD to the raw data, the extracted features, and the concatenation of the two, picking, for each, the combination of LMFT parameters and the `penalty' parameter that produces the highest F1-score.
\end{enumerate}
%
 The validation process is as follows:
%
\begin{enumerate}
 \item Using the parameters chosen by the training procedure, apply local GPR to all channels of each validation sequence, obtaining a new sequence of LMFT features.
 \item Using the penalty parameters chosen by the training procedure, apply PELT to the validation set raw data, the LMFT features and the concatenation of the two.
 \item Compare the results in terms of the confusion matrices, precision, recall and F1 score.
\end{enumerate}
%

\subsubsection{EEG Epilepsy Data} \label{section:eegmethodology}

Finally, we provide an analysis of algorithm performance on the task of epilepsy detection from EEG readings.
 A dataset of 39 eeg recordings each involving an epileptic event was obtained from the authors of \cite{luckett2017dissimilarity}.
 Recordings are in the 10-20 international system, resulting in 21 channels of unfiltered surface EEG signals sampled at 250Hz.
 The approximate point at which the epilieptic event occurs is also noted.

Since EEG recordings are notoriously noisy, we have preprocessed the data in an attempt to clean up some of these artifacts.
 We have followed advice from \cite{gil2012electroencephalography} in reviewing the raw signals.
 Firstly, the Fourier spectrum of a nonepileptic section of an arbitrarily chosen channel of data was reviewed and can be seen in Figure \ref{figure:fouriereeg}.
 Note the prominent spike around 60Hz corresponding to what is likely contamination from mains hum.
 In order to reduce the influence of these artifacts, we apply a filter with both low and high pass components.
 The applied filter's Fourier spectrum is shown in Figure \ref{figure:kumaraswamyfilter}, and is designed to accentuate signals in the ranges of `ordinary' neural activity, and possibly muscle spasms.
 The filtered Fourier spectrum from Figure \ref{figure:fouriereeg} is shown in Figure \ref{figure:filteredfouriereeg}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{raw_fft_eegDAT.F00012}}}
    \caption{The Fourier spectrum of a channel of EEG recordings.}
    \label{figure:fouriereeg}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{kumaraswamy_filter_a01.20_b10.00}}}
    \caption{The Fourier spectrum of the filter applied to the EEG recordings.}
    \label{figure:kumaraswamyfilter}
\end{figure}
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{kumaraswamy_filtered_fft_eegDAT.F00012_a01.20_b10.00}}}
    \caption{The Fourier spectrum of the filtered EEG recordings.}
    \label{figure:filteredfouriereeg}
\end{figure}

After filtering the data, we subsample the data for computational efficiency to reduce the sample rate to 50Hz.
 Since most of the high frequency signals have already been removed, there is no good reason to retain a high sample rate.
 Note that it is important to filter the recordings \emph{before} subsampling, since otherwise there may be aliasing from the mains hum at a lower frequency.
 
From visual inspection of the signals, non-normal eeg signals appear within less than a minute of the recorded event time.
 Thus, we propose to analyze 200s long fragments of each recording.
 \cite{gil2012electroencephalography} suggest that frontal lobe seizures do not typically last for multiple minutes, so that 200s of signal should be sufficient to capture both a period of nonictal and ictal activity.
 39 `positive' fragments are taken to include 100s of eeg signals before and after the label of the epileptic event.
 39 `negative' fragments are taken to include 200s of eeg signal sampled during a section equidistant from the beginning of the recording and the noted time of the epileptic event.
 Each recording is at least an hour long, so this results in a balanced dataset containing signals representative of the onset of an epileptic event and signals representative of ordinary neural activity.

We propose to extract local GPR features from each channel of an eeg recording, resulting in a $N_t\times N_c \times N_f$ tensor, where $N_t$ is the recording length, $N_c$ is the number of channels (21), and $N_f$ is the number of features extracted from each channel.
 We then flatten the last two axes to re-obtain a time-series of vectors allowing traditional analysis, resulting in a transformed dataset of shape $N_t\times N_cN_f$.
 
Brainwaves are often interpreted in terms of their various length scales, with delta waves on the order of 0.5-4 Hz, up through beta waves at 12-30 Hz and including other, even higher frequency waveforms.
 Our downsampled data is incapable of revealing any frequencies above the beta range.
 In addition to altered brainwave patterns, ictal activity is sometimes associated with motor activity, which is on the order of delta waves or somewhat lower \cite{gil2012electroencephalography}.
 
In order to detect changes in these various brainwave patterns, we employ a GPR covariance function of the following form:
%
\begin{equation} \label{equation:eeggpr}
    C_{\text{eeg}} = CN_c RBF_r + WN_w
\end{equation}
% 
 The $CN * RBF$ component is designed to model changes in brain wave activity and also motor activity.
 In order to constrain the model to detect such changes, we fix the $RBF$ term with a length scale $l$ representative of delta waves.
 We accomplish this by fitting an unconstrained GPR with the above covariance function to a simple sine wave with a period in the delta wave range, and a scale comparable to the EEG signals.
 We further fix the $WN$ term with a noise level at $1$, large enough to encourage the covariance matrix to be positive definite, but small enough to have a relatively small effect on the model.
 To see that this should have a small effect on the model, we note that the scale of the signals is on the order of hundreds of units.
 We further note that our low-pass filter preprocessing step removes most of the signal that might be considered white-noise, and so fixing the white noise level to be rather low is not unreasonable.

By fixing the parameters of the $RBF$ terms, we hope to interpret the locally-trained parameters of the \emph{CN} term as representing changes in the pattern of brain waves or of motor activity.
 We hypothesize that the features so extracted will be useful in the detection of the onset of epileptic events.

As discussed in Section \ref{section:contrivedresults} the optimization surface for GPR (Equation \ref{equation:gprobjective}) is often highly non-convex and is thus very sensitive to starting parameters.
 This has the effect of creating instability in the learned parameters over time, as previously observed values exit the model and new values enter.
 In order to partially account for this, we first fit an `exemplar' model to an arbitrary section of signal from a non-ictal region.
 The exemplar model is fit using 400 initial seeds to obtain approximately globally optimal parameters.
 The trained model parameters of the exemplar model are then used to seed the starting parameters during local model training.

In order to classify a fragment as containing ictal activity or not, we will observe changes in the extracted local GPR features.
 Specifically, we anticipate that the extracted features will be significantly different depending on whether the query time is during or near an ictal period.
 However, we hypothesize that the complex patterns exhibited by ictal activity in the raw signal will translate to simpler patterns in the extracted features.
 We anticipate that this will improve the power of classical methods used to classify arbitrary time series.

We propose, therefore, to employ 1NN with DTW variously on the raw signals, on the LMFT-extracted features, and on the concatenation of the two.
 We split the above-described dataset of segments representing both non-ictal activity and those representing the onset of ictal activity $\sim 50/50$ into train ($n=20$) and validation ($n=19$) sets.
 We then classify the validation set by 1NN with DTW against the training set.
 We will then evaluate the results of the three possibilities by comparing the confusion matrices, and particularly precision, recall and accuracy.

DTW is based in part on calculating a Euclidean distance between points at similar times.
 Therefore, it is sensitive to the relative scale of the various features, and features with smaller scales are effectively weighted down in importance.
 Therefore, in order to effectively apply DTW to the concatenation of the raw data with the extracted features, we scale each channel and each feature to have mean 0 and standard deviation 1.
 Since the various channels of the raw data are all of a comparable scale, and so too with the extracted features, we do not perform any scaling when applying DTW to only raw data or only extracted features.

% Thus, instead of attempting to predict the exact pattern of local model features associated with ictal activity, we will merely look for a significant difference in the extracted features.
% This can, in theory, be accomplished by disregarding the time variable and applying out-of-the-box unsupervised clustering algorithms for which the number of clusters is not chosen a priori.
% We will employ the Mean-Shift \cite{comaniciu2002mean} algorithm, both because it fits the above description and also because it is, itself, a type of local modeling algorithm.
% Since we expect the samples containing epileptic activity to consist of both ictal and nonictal signals, we might expect that these signals would contain more than one cluster of extracted features.
% On the other hand, samples not containing epileptic activity should only consist of a single cluster.

%We employ the tricube kernel for this mean-shift step as well (Equation \ref{equation:tricube}) and choose the bandwidth in such a way that the training sample with epileptic activity robustly gives 2 clusters.
% Specifically, for kernels with non-finite support such as the Gaussian kernel, as the bandwidth $\rightarrow \infty$, the Mean-Shift algorithm will result in a single cluster.
% As the bandwidth $\rightarrow 0$, the Mean-Shift algorithm will result in a single cluster for each data point.
% Although the number of clusters is not continuous in the bandwidth, this suggests that there might be a range of bandwidths that tend to result in exactly 2 clusters.
% In practice, it has been our observation that this intuition plays out, even when using a kernel with finite support such as the tricube kernel.
% In any case, we apply Mean-Shift for a variety of bandwidths, and select an optimal bandwidth $b_{\text{MS}}$ that lies at the median of all bandwidths resulting in 2 clusters.
% We would thus expect that data which results in multiple clusters contain ictal activity, and data which results in a single cluster does not.
% Note that it would be possible to construct a ROC curve against possible values of $b_{\text{MS}}$ employing this desideratum, since large values would result in a $100\%$ negative rate, and small values would result in a $100\%$ positive rate.
% However, the small size of our dataset has rendered this infeasible.
 
Since the dataset is quite small, we set aside 2 of the training samples for selection of the kernel bandwidth $b_{\text{GPR}}$ for the local GPR models, and also for selection of fixed parameters in the covariance function.
 Our process of `training' to obtain these hyperparameters consists of visualization of the extracted signals for various setting and also a priori knowledge of the nature of the data.
 Note that in the presence of additional data, it might be possible to train over available bandwidths to obtain an optimal one for the task at hand (differentiating ictal vs non-ictal signals).
 The possibility of automating training is reserved for future investigations, and the subjectivity inherent in our training procedure is a limitation of the current research.

To summarize, the data preprocessing steps, applied to all data, are as follows:
%
\begin{enumerate}
 \item Filter data using the filter in Figure \ref{figure:kumaraswamyfilter}
 \item Downsample data to 50Hz
\end{enumerate}
%
 The training process is as follows:
%
\begin{enumerate}
 \item For various bandwidths, apply local GPR to all channels of the training eeg.
 \item Visualize the extracted features, choosing an optimal bandwidth $b_{\text{GPR}}$, and an optimal value for the RBF term parameter $r$ that together seem to result in the strongest desired signal.
\end{enumerate}
%
 The validation process is as follows:
%
\begin{enumerate}
 \item Using the bandwidth $b_{\text{GPR}}$ and $r$ chosen by the training procedure, apply local GPR to all channels of each validation eeg.
 \item For the raw data, the extracted features, and the concatenation of the two, apply 1NN with DTW to classify the validation eegs.
 \item Compare results via their respective confusion matrices.
\end{enumerate}
%


==> local_gpr/results/long_results.tex <==

\section{Results} \label{section:results}

\subsection{Contrived Data} \label{section:contrivedresults}

In this section we investigate a number of practical issues related to obtaining local modeling with Gaussian Processes, including the stability of features over time, hyperparameter selection, and the interpretation of any extracted features.
 We use these initial investigations to inform the setup for later experiments.

\subsubsection{Stability of Extracted Features} \label{section:stability}

At a very basic level, in order for features extracted from a dataset to provide any meaningful insight into the dataset, they should be non-random, and should vary more-or-less continuously with the time-series under consideration.
 By more-or-less continuously, we note that, for example, change point detection algorithms produce non-continuous output in the form of a point-impulse at various locations.
 However, the number of discontinuities in the signal output by a change point detection algorithm are relatively few, and the output features are almost everywhere 0 (indicating no-change).
 On the other hand, features that consist of a very large number of large jump discontinuities are probably not helpful.
 We note this because the algorithm described in Section \ref{section:algorithm} is not mathematically guaranteed to provide stable output.

However, by experiment we show that, by appropriate choice of hyperparameters and other factors, we can encourage a sufficient amount of stability in the extracted features.
 In the remainder of this section, we will explore the underlying mechanisms which might cause instability in the output of the algorithm, and to then propose ways that we might mitigate these issues.

In general, for kernel methods, a smooth kernel gives a smoothly varying optimization surface at each point in time, which results in a smoothly varying optimum over time.
 However, this helpful property does not apply for us, because of the fact that the optimization surface of a GPR is not generally convex.
 Therefore, our algorithm may exhibit discontinuities depending on a variety of factors.
 These include, but are not limited to the choice of seed for the optimizer at each point in time and the number of parameters available to our chosen covariance function.
 Regardless of how we might choose a seed for our optimizer, or various other considerations, however, the output of the algorithm cannot be guaranteed to be continuous.

Before continuing, we would like to examine the continuity claim above that we would have if the optimization surface \emph{were} convex.
 For mathematical simplicity, we only consider here loss functions of the following form, which is a very common form:
%
\begin{equation}
 L(X,\theta,q) = \sum_{x\in X} l(x,\theta)K(x,q)
\end{equation}
%
 Where $X$ is our dataset of size $n$, $l(x,\theta)$ is a bounded loss for a single point $x$, given parameters $\theta$, and $K(x,q)$ is the weight at point $x$ given a query point $q$.
 We are specifically concerned with local weighting schemes, and we will ask what happens to this total loss as the query point changes by a small amount.
 Suppose then, that we have some small quantity in mind, $\delta > 0$ and that $|l(x,\theta)| < M$.
 If $K$ is continuous and symmetric, then we can choose $\epsilon>0$ so that $|K(x,q')-K(x,q)| < \delta/(nM)$ for a given $x$ whenever $|q-q'|<\epsilon$.
 This implies that $|L(X,q',\theta) - L(X,q,\theta)| < \delta$, so that the total loss is also continuous in $q$ at any given $\theta$.
 Our requirement that $l$ be bounded amounts to a bound on $\theta$, but since our dataset $X$ is fixed, this is not an unreasonable requirement for most model families.
 
We would like to see that the optimal parameters $\theta_\text{opt}(q)$ that minimize the total loss at $q$ are also continuous in $q$.
 Choose another $\delta > 0$.

First, observe that for any $\delta > 0$ we can choose an $\gamma > 0$ so that:
$$ \begin{array}{l}L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 This can be acheived by simply setting $\gamma$ so to be the minimum difference $L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q))$ for all $\theta''$ so that $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 To show the contrapositive, choose a $\theta'$ so that $|\theta' - \theta_\text{opt}(q)| > \delta$.
 Choose $\theta''$ to be the point so that $\alpha \theta' + (1-\alpha) \theta_\text{opt}(q) = \theta''$ where $|\theta'' - \theta_\text{opt}(q)| = \delta$.
 Since $L(X,q,\theta)$ is convex in $\theta$ for a given $q$ then:
$$L(X,q,\theta'') < \alpha L(X,q,\theta') + (1-\alpha) L(X,q,\theta_\text{opt}(q))$$
 This gives:
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) \\ > (L(X,q,\theta'') - L(X,q,\theta_\text{opt}(q)))/\alpha \\ > \gamma/\alpha > \gamma \end{array} $$
 
This shows that all of the points $\theta$ that have a ``small" loss are near the current $q$'s optimum.
 We will now combine this fact with $L$'s continuity in $q$ to acheieve the desired result.
 Pick $\gamma > 0$ so that 
$$ \begin{array}{l} L(X,q,\theta') - L(X,q,\theta_\text{opt}(q)) < \gamma \\ 
   \rightarrow |\theta' - \theta_\text{opt}(q)| < \delta \end{array}$$
 Further restrict $\gamma$ so that 
$$ \begin{array}{l} L(X,q',\theta') - L(X,q',\theta_\text{opt}(q')) < \gamma \\ \rightarrow |\theta' - \theta_\text{opt}(q')| < \delta/2 \end{array}$$
 Pick $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ \begin{array}{l} 0 < L(X,q',\theta_\text{opt}(q) - L(X,q,\theta_\text{opt}(q) = \\ |L(X,q,\theta_\text{opt}(q)) - L(X,q',\theta_\text{opt}(q))| < \gamma/2 \end{array}$$
 Further restrict $\epsilon > 0$ so that $|q-q'| < \epsilon$ implies 
$$ L(X,q,\theta_\text{opt}(q')) - L(X,q',\theta_\text{opt}(q')) < \gamma/2$$
 Combining the previous two facts, we have $|q-q'| < \epsilon$ implies 
$$\begin{array}{l} (L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q))) + \\ (L(X,q',\theta_\text{opt}(q) - L(X,q',\theta_\text{opt}(q'))) < \gamma \end{array}$$
 Since $L$ is optimized at $\theta_\text{opt}$, both of these terms are positive, and we have that $L(X,q,\theta_\text{opt}(q')) - L(X,q,\theta_\text{opt}(q)) < \gamma$.
 This implies that $|\theta_\text{opt}(q) - \theta_\text{opt}(q')| < \delta$, which gives the desired result.

In other words, if the optimization surface is convex, then new time series formed by extracted parameters will be continuous.
 If the model family consists of continuous functions, this will further imply a continuous sequence of predictions, which is why LOESS gives continuous curves.
 However, if the optimization surface is \emph{not} convex, then no such continuity is guaranteed.
 Such discontinuities might occur even if the optimization surface is smooth.
 This means that as our time series progresses, the extracted model parameters may experience discontinuities, and these discontinuities are not necessarily related to anything special happening in the data.
 We show this by counterexample.

In Figure \ref{figure:discontinuousoptimaneighboringbeta0}, we show potential loss surfaces over which we intend to optimize a parameter displayed on the $x$ axis.
 Imagine that, as we change $q$, the optimization surface changes at each time step from the function at top to the function at bottom.
 At the top, the loss surface contains a single minimum, which our optimization procedure finds.
 If we seed a gradient descent optimizer with the previous time steps optimum, we will find the points in red.
 Note that this point changes continuously until the local optimum at that point disappears, at which point the optimizer slides to an entirely new local minimum elsewhere.
 The point at which this local minimum disappears will create a discontinuity in the extracted parameters.
 In the case that we use an optimizer that is capable of finding the global minimum at each point, there will be a discontinuity in the optimum at the middle function ($h=1,k=-1$), at which point the two optima have an equal loss.
 In the case that we use a gradient descent optimizer seeded with a constant value, it will experience a discontinuity, but it is not clear at what point that discontinuity will occur.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_neighbor_beta0}}}
    \caption{The family of functions $3x^4-4(k+h)x^3+6khx^2$ for varying values of $h,k$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the previous time-steps optimum.}
    \label{figure:discontinuousoptimaneighboringbeta0}
\end{figure}

Worse, if we seed a gradient descent optimizer with a constant value, the local optima need not disappear in order to experience a discontinuity.
 In Figure \ref{figure:discontinuousoptimaconstantbeta0}, we can see that such a thing might happen.
 Note that this observation also holds for a robust global optimizer that finds the global optimum.
 In the same figure, the two displayed optima have the same loss value, so that a global optimizer might jump between these two values due to small fluctuations.
 Thus, we expect a good global optimizer to actually give \emph{less} stable results than a simple gradient descent optimizer with an appropriate seed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{disappearing_minimum_fixed_beta0}}}
    \caption{The family of functions $(x-h)^4-2(x-h)^2$ for varying values of $h$.
    The red dots illustrate the optima found under a strategy of seeding a gradient descent optimizer with the seed at the orage vertical line.}
    \label{figure:discontinuousoptimaconstantbeta0}
\end{figure}

Lastly, we note that, even if a gradient descent optimizer seeded with the previous time-steps optimum does not experience a discontinuity due to the disappearance of the previous time-step's optimum, the local optimum may become very sub-optimal over time.
 Worse, the series of extracted parameters can therefore become `stuck' at a poor local optiumum, and may remain there for the entire time series.

So, we see that when the optimization surface is not guaranteed to be convex, the extracted features cannot be guaranteed to be continuous.
 However, the strategy by which we seed the optimizer can have an effect on the stability of the results.
 We consider here, empirically, the 3 optimizer strategies discussed above: constant seed, seed with neighboring interval optimum value, and global optimization.

All of these options can be seen in practice in Figure \ref{figure:contrivedvariancevariousfixedparameters}, displaying results from the various seed strategies, and also for various selections for fixing covariance function hyperparameters, which we discuss later in this section.
 In each of the graphs in Figure \ref{figure:contrivedvariancevariousfixedparameters}, the constant term and RBF term parameters are fixed to various values, and the optimizer for the remaining white noise term $w$ is seeded according to various strategies.

In the third set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we simply seed the the optimizer with a starting value that is equal to the fixed constant term value used for that set of features. 
 This seed is employed at every point in time.
 In the 1st and 5th graph down, we can see that some choices of hyperparameters can result in an unstable set of features.
 However, in the 2nd, 3rd and 4th graphs, we can see that a good choice of hyperparameters can result in a more stable set of features.

In the second set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters} we seed the optimizer with the optimum found at the previous point in time.
 We can see in 1st and 3rd graphs that, although the extracted parameters seem to pick up on the change in white noise level, they do not readily return to `normal' levels after the period of altered noise.
 This suggests that they have become `stuck' at a suboptimal local minimum.
 Worse, the 1st, 3rd and 5th graphs suggest that the strategy of seeding the optimizer with a neighboring query point's optimal parameters is not as helpful in encouraging stability as we might have hoped.

In the top set of features of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we seed the optimizer with both the previous time step's optimal parameters and also the exemplar period.
 If the optimum found by seeding with the exemplar parameters has a higher marginal likelihood than at the optimum found by seeding with the neighboring optimum, we fit a GPR with hundreds of seeds spread log-uniformly throughout the parameter space.
 This emulates fitting an optimizer capable of finding the global optimum.
 It is clear that fitting a global optimizer is even more unstable than fitting an optimizer with a fixed seed.
 We suspect that this is because, with a fixed seed, the optimizer can only find local optima "near" the seed.
 However, with a global optimizer, we can find the global optimum no matter where it should appear in the search space, so there is more opportunity for the optimum to switch.
 In any case, it seems that in practice, the global optimizer creates highly unstable results.
 This is just as well, because seeding an optimizer with hundreds of seeds is incredibly time-consuming, and results in a significantly less efficient process.

Furthermore, for various covariance functions and data, the sought-after optimum might be in a very "narrow" valley.
 To the point that finding it using a random seed is a rather unlikely event, and so a great number of seeds must be employed to reliably find good optimal paramter estimates.
 This is illustrated in Figure \ref{figure:contrivedperiodgpr}.
 These parameters are extracted by training over the constant and period paramters and fixing the length scale and white noise parameters in Equation \ref{equation:variableperiodcovariance}.
 100 random seeds are chosen log-uniformly on $[10^{-10},10^{10}]$ and the optimizer is run on each of these, with the best result taken in the end.
 Approximately half of the time, a period on the order of tens is found, which is representative of the approximate period of the local data at that point.
 Figure \ref{figure:contrivedperiodgprsmooth} shows a Nadarya-Watson-smoothed version of the curve in Figure \ref{figure:contrivedperiodgpr}.
 Note that the period generally increases toward the middle of the data, and decreases toward the edge, which is reflective of the properties of the underlying data.
 However, the "correct" optimum can be difficult to find, especially for periodic covariance functions where one might reasonably expect a local minimum at factors of the "true" period.
 The result is unstable local parameters over time.

From these observations, we believe that seeding the optimizer with a fixed set of parameters that are near a "normal operating" value to be a good partial solution to the discontinuity problem.
 The proceeding experiments will therefore all employ this option.

Another strategy that can be employed to increase the stability of the results is to reduce the size of the parameter space.
 Specifically, we would a priori expect that an optimization surface over many variables would have more opportunities to play host to superfluous local optima than an optimization surface over fewer variables.
 One way to accomplish this is by `fixing' some of the parameters in the covariance function at convenient values to allow analysis only of parameters of interest.
 Fixing the parameters of the individual models has other side-effects on the model in addition to affecting the stability of the algorithm.
 It is worth noting that a `fixed' parameter essentially becomes a hyperparameter of the algorithm that must be set by some means besides the ordinary training scheme.
 We therefore discuss these effects in the proceeding section

\subsubsection{Setting Hyperparameters} \label{section:hyperparameters}

Similarly to LOESS or kernel density estimation, we must set a kernel bandwidth.
 There has been a great deal of work into bandwidth selection, with a number of reviews covering the subject, for example \cite{turlach1993bandwidth}.
 The effects of bandwidth selection have mostly been considered in relation to local model predictions.
 However, since predictions are generally a function of the parameters, the sundry factors largely translate to the problem at hand.
 Since our datasets contain relatively little data with which to train this hyperparameter, we set it naively using a priori information concerning the nature of our datasets, and do relatively little to explore its effects.

The remaining hyperparameters consist of any fixed parameters in our covariance functions.
 Fixing the parameters in our covariance function may seem to be a strange step from the point of view of attempting to accurately model the data, so we discuss it briefly here.
 We remind the reader that \emph{our purpose here is not to model the data as accurately as possible}.
 Instead, we aim to extract features from the data for an entirely different purpose than interpolation or extrapolation.
 Therefore, the model most suited to interpolation or extrapolation may or may not be the model best suited to our needs.
 Still, any arbitrary model will not do, and we need a ``well-fit" model in some sense.
 It is important to realize that that sense is some combination of the ordinary sense of fitting models (interpolation and extrapolation) but also the extraction of features best suited for whatever the ultimate use of our features will be.
 Such use cases may include change point detection, as in Section \ref{section:accelerometrymethodology}, time series classification, as in Section \ref{section:eegmethodology} or others.

We note that there are 3 "levels" at which we can allow the various parameters to vary.
 At the highest level, allowing it to vary maximally, we could allow a parameter to be trained in the individual local models.
 At this level, a parameter is simply an additional feature extracted from the time series.
 At a middle level, we could fix the parameter during portions of a sequence, or for a single sequence in a group of sequences, but allow it to vary between sequences
 At the lowest level, we could fix the paramter once for the entire sequence or for all sequences in a group using information gleaned from a set of training sequences.
  
The highest level has the ostensible benefit of providing an additional feature that can be used for learning at a later stage.
 It also benefits from the existence of a pre-existing tried-and-true training method, since they would be obtained from the locally-trained GPRs.
 Lastly, it benefits from the ability to show variation in this parameter between different individuals.
 However, this can result in features that are less stable over time, as the optimizer finds various transient local optima.
 A second pitfall is that the various parameters are not independent.
 In other words, we will obtain a different sequence of white noise term parameters depending on whether we fix the constant term and RBF term parameters or not, and will obtain different sequences depending on what levels we fix them at.
 Both of these problems can be witnessed in Figure \ref{figure:allvarscontrivedvariance}.
 It is therefore not clear that the white noise term sequence will benefit from the additional parameter, and in our experience on this and the accelerometry dataset it does not.

The lowest level solves the problems at the highest level associated with learning multiple parameters.
 It may also help alleviate some of the dependence between parameters during GPR training.
 However it suffers from not allowing variation between individual sequences in a group.
 It is also disadvantaged by ignoring potentially valuable information from an additional extracted feature.
 It also requires the creation of a method for choosing an appropriate fixed parameter.
 However, it is not clear that the additional feature is, in fact, useful: recall the previous discussion concerning the distinction between the best parameters for interpolation vs that for activity recognition.
 If we are specifically interested in one particular parameter, and expect relatively little variation in the scale of other parameters between groups, this option may be best.
 In the third set of graphs of Figure \ref{figure:contrivedvariancevariousfixedparameters}, we can see that this plays out.
 In the contrived variance dataset, although there is some change in, e.g., the curvature of the function over time, which may reflect in the learned parameters, the primary feature of change is the noise level.
 By fixing the other parameters at a convenient level, we can focus the method onto changes in one particular variable, control for the dependence between the parameters, and ease the number of discontinuities in the extracted features over time.
 Specifically, the third graph seems to extract the desired signal from the data very well, giving a large value when the noise level is large, and a small value when the noise level is small.

The middle level also solves the problems at the highest level associated with learning two parameters.
 It also has the benefit of allowing a variation in "baseline" readings between individuals.
 Like the lowest level, it may be disadvantaged by losing an additional feature.
 Similarly, it requires the creation of a method for choosing an appropriate fixed parameter.
 Since the parameter is fixed individually for a sequence, the method devised above for choosing a fixed parameter cannot apply if we cannot depend upon having labelled data for every individual.
 One option may be to train a GPR with the parameter allowed to vary on an exemplar segment of data chosen at random from the sequence, and then to subsequently fix the parameter in the local model training to be the value obtained from the exeplar segment.
 This would solve the problem of optimization surface complexity from the highest level.
 However, it would still suffer from having a parameter chosen for the purpose of interpolation rather than activity recognition.
 Furthermore, there is no guarantee that our `exemplar' segment is, in fact, exemplary.
 Since the contrived data do not involve a great deal of variation in the signal, and do not involve signal from multiple individuals, we do not explore this option here.
 Instead, we include discussion related to this possibility with respect to the accelerometry data, we direct the reader to Section \ref{section:accelerometryresults}, and with respect to the eeg data to Section \ref{section:eegmethodology}.












 Indeed, for this dataset, does an "exemplary" segment come from a sequence where a subject was sitting or walking?
 Still, since it not unreasonable to expect that the best parameter for interpolation might yet be a quite good parameter for other purposes, we investigate this method of setting the constant term parameter as well in Section \ref{section:accelerometerresults}.






Note the length scales of the x-axis in Figure \ref{figure:chestaccelerometerZMinutes}.
 Although the signal appears to have a very prominent noise component when viewed at a resolution on the order of minutes, it is significantly less noticeable when we zoom in to see changes at the level of seconds, as seen in Figure \ref{figure:chestaccelerometerZSeconds}.
 This is because there is meaningful small-scale structure to the accelerometer readings.
 However, that small-scale structure is not necessarily useful in distinguishing between various activities.
 In fact, note that the data in Figure \ref{figure:chestaccelerometerZSecondsfixedrbf} is taken during a single activity, suggesting that a good extracted feature for this data should approximate a constant value indicative of the present activity.
 Allowing the optimizer to choose the parameter of the RBF component of our covariance function may therefore not be an optimal method for extracting the noise component.
 Worse, it is possible for the RBF component to, itself, model white noise.
 Specifically, as the length scale of the RBF component goes to 0, the $CN_c RBF_r$ term simply becomes an $WN$ component.
 It is therefore difficult to prevent interactions between these two terms when optimizing our individual local models.
 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr}}}
    \caption{An example taken from the chest accelerometry dataset, showing data on the scale of seconds.
        All parameters in the GPR covariance function (Equation \ref{equation:accelerometergpr}) are allowed to vary.
        400 log-uniform seeds are chosen to obtain globally-optimal parameters.
        The optimal RBF length scale is found to be $\approx 0.33s$.
    }
    \label{figure:chestaccelerometerZSeconds}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometry_exemplar_gpr_fixed_r}}}
    \caption{The same data from Figure \ref{figure:chestaccelerometerZSeconds}, but with a fixed RBF length scale parameter at $\approx 15s$
        The remaining parameters are allowed to vary.
    }
    \label{figure:chestaccelerometerZSecondsfixedrbf}
\end{figure}



Since we are primarily interested in the noise level term parameter, we further have the constant term parameter to contend with.
 In Section \ref{section:accelerometerresults}, we provide some exploratory investigation into allowing it full freedom to vary along each time series or fixing it to be a particular value for the entire experiment.
 However, as we have noted, there is a strong interaction between the two additive terms in our covariance function.
 Therefore, we have chosen to fix the constant term parameter as well, at a level convenient for change point detection, chosen by manual inspection of the extracted signals.
 Changing the constant parameter has an effect on the sensitivity of the extracted signal, and also on the stability of the extracted signal.
 Low values give a highly unstable signal.
 High values make the feature extraction insensitive to changes in variance, resulting in a "flat-line" for extremely large values.
 An example set of extracted features, where the hyperparameters are chosen to give a good signal by visual inspection, are seen in Figure \ref{figure:accelerometer5}.
 
Indeed, this is exactly the reason why we fixed the \emph{RBF term} parameter.
 Fixing the constant term parameter, however, is not as straightforward as choosing the RBF term paramter.
 Firstly, the more parameters we fix, the more opportunity there is to constrain our model family in such a way that it cannot possibly give a "good" model.
 Secondly, The units of the RBF term parameter are easily interpretable and therefore lend themselves to being fixed according to our a priori conceptions about the data.
 The optimal constant term parameter is related to the overall variance in the signal, but it also depends on the RBF term parameter, and we therefore lack the insight to simply fix it based on our expertise in the subject.
 Although we cannot set it a priori, it seems reasonable that we might simply train this parameter against a training set of accelerometer readings to optimally predict the true labels.
 We investigate such a procedure in Section \ref{section:accelerometerresults}.





First, there are a number of hyperparameters affected execution of the algorithm.
 Recall from Section \ref{section:accelerometrymethodology} that we have an option to fix various parameters of the GPR during local model training.
 If we elect to fix any of the model parameters, the value at which they are fixed can be considered a hyperparameter of the local model feature extraction.
 Lastly, we need to set the bandwidth for our kernel.
 We will investigate here the effect of all of these various hyperparameters on the results of the algorithm, as well as the effects of fixing the various parameters in the local models.
 Instead of providing a full grid over the various hyperparameters, we will take pick and choose what we consider to be representative possibilities that illustrate possible pitfalls and prospects of local model feature transformations with GPR.

One factor compounding the issue of discontinuous local parameters over time is the dimensionality of the parameter space.
 The larger the space, the more opportunity exists for local optima to appear and disappear, and to generally move up, down and around one another over time.
 Thus, if we identify target parameters that we expect to be indicative of particular properties of interest in our time series, we can potentially "fix" the other parameters.
 This potentially has two advantages.
 First, the size of the parameter space is reduced, potentially improving stability of extracted parameters over time.
 Second, problems with interpreting changes in the local parameters due to dependence between the various parameters is reduced, since only a limited set of the parameters are allowed to vary.
 In other words, changes in a non-target parameter do not cause changes in the target parameter, since the non-target parameter is simply not allowed to vary. 
 We direct the reader to Section \ref{section:accelerometrymethodology} for a more thorough discussion of how "fixing" certain parameters is expected to affect the overall procedure.

Figure \ref{figure:contrivedvariancevariousfixedparameters} shows the results of training a local GPR on our contrived dataset while fixing the RBF term and the constant term's parameters (see Equation \ref{equation:variablevariancecovariance}).
 We seed the white noise parameter with a value of $1$ at all points in time, although we note that the particular seed value used does not much affect the results, so long as the seed is fixed.
 
We will here attempt to explain the extracted features in terms of the intuition behind the chosen form of the covariance function.
 This will provide us with a basis for setting the model parameters in future iterations.
 We note that, although these explanations are based largely on the intuitions outlined in \cite{rasmussen2005gaussian}, they are otherwise post hoc.
 Therefore, these explanations should be taken to be hypothetical.
 Although we will not test them directly, we employ them implicitly in constructing later models, and the reader can weigh the evidence for these explanations in part by the procedure's performance on these subsequent experiments.

 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{illustrative_pairs_contrived_variance}}}
    \caption{Variable noise data below in orange.  
    The three sections divided by a horizontal black line are: top - global parameter search, middle - neighboring parameter seed, bottom - fixed parameter seed.
    Within each section, the graphs in blue represent local GPR white noise parameter freatures obtained with fixed $c,r$ at various values.
    From top to bottom, within each section, the $c,r$ pairs are: $(32,8),(64,2),(64,512),(.25,.12)$ and $(.25,2)$}
    \label{figure:contrivedvariancevariousfixedparameters}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{all_vars_contrived_variance}}}
    \caption{Variable noise data below in pink.
        The other graphs represent the various parameters of a locally trained GPR over time.}
    \label{figure:allvarscontrivedvariance}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr}}}
    \caption{Variable period data below in green.
        Extracted gpr parameters are period for the exponential sine squared term in orange, and the constant term value in blue.
        100 seeds are chosen log-uniformly on $[10^{-10}, 10^{10}]$.}
    \label{figure:contrivedperiodgpr}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{contrived_period_gpr_smoothed}}}
    \caption{The same extracted features from Figure \ref{figure:contrivedperiodgpr}, but smoothed by a weighted rolling mean. 
    }
    \label{figure:contrivedperiodgprsmooth}
\end{figure}


 

\subsection{Accelerometry Data} \label{section:accelerometerresults}

%TODO the transformed data are in chest_acc_run019/transformed_data

In this section we discuss the results of the proposed feature extraction algorithm applied to the accelerometry dataset described in Section \ref{section:accelerometrymethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on discovery of change points in time series.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the signals from 2 different individuals.
 A portion of the signal containing the ground truth change points for both sequences can be seen in Figures \ref{figure:accelerometer5} and \ref{figure:accelerometer6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:accelerometrymethodology} is also shown.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_05_y_axis}}}
    \caption{y-axis acceleration from one of the sequences in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{accelerometer_06_z_axis}}}
    \caption{z-axis acceleration from a second sequence in the accelerometry data.
        Above is the extracted set of features from the learned white noise parameter of a local GPR.}
    \label{figure:accelerometer6}
\end{figure}

The hyperparameters used in these graphs were chosen from a log-uniform grid search to return the maximum signal upon visual inspection.
 Although we do not include the full results of the grid search, we refer the reader to Section \ref{section:contrivedresults}, and specifically Figure \ref{figure:contrivedvariancevariousfixedparameters} for comparable results on the contrived datasets.

In Section \ref{section:eegmethodology} we describe a process by which an exemplar model may be used to obtain the seed values for local model training.
 However, this process was not found to be effective for the accelerometry dataset. 



\subsubsection{Confirmatory Results}



\subsection{EEG Epilepsy Data} \label{section:eegresults}

In this section we discuss the results of the proposed feature extraction algorithm applied to the eeg dataset described in Section \ref{section:eegmethodology}.
 We provide both insight into the problem by means of our initial exploratory investigations and also the results of the confirmatory experiments based on classification of subsequences of the data.

\subsubsection{Exploratory Results}

Our initial explorations of the proposed feature extraction method on this data focused primarily on the positive (including ictal onset) subsamples from 2 different individuals.
 The positive samples contain both ictal and non-ictal activity, and were expected to therefore illustrate the differences in the extracted features for these two types of eeg signals.
 A portion of the signal containing the labeled point of ictal onset for both sequences can be seen in Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6}.
 The extracted features corresponding to the local model feature extraction procedure detailed in \ref{section:eegmethodology} is also shown.
 Some caution is advised in the interpretation of these graphs, since these are our `training' data, and parameters have therefore been specifically selected in such a way as to obtain a `nice' signal.

Some other configurations of hyperparameters were attempted, but did not give pleasing results.
 Notably, in early experiments we attempted to model the data locally using a covariance function with 4 RBF terms.
 Each was set at a length scale corresponding roughly to the various waveforms commonly encountered in brain activity - beta, alpha, theta and delta waves, and the constant value term was allowed to vary locally.
 However, in experiments, the features extracted at the various length scales were highly correlated, resulting in superfluous features.
 Furthermore, the correlation resulted in a situation where the signal represented by one term overlapped sufficiently with the other terms as to frequently cause a deep local optimum at 0 for the other terms.
 It was therefore often the case that one term would dominate, and the resulting signal was highly unstable with the various terms going to 0 at different times.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00019_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from one of the recordings, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset5}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{static/{{F00020_ictal_onset_gpr_illustrative}}}
    \caption{Approximately 60s of channel FP1 from a second recording, filtered and including the labelled point of ictal onset.
        Above is the extracted set of features from the learned constant value parameter of a local GPR.}
    \label{figure:ictalonset6}
\end{figure}

Due to these issues, the single-term configuration was chosen for improved stability at the expense of interpretability.
 We did not experiment with a wide variety of RBF length scales, since the scale characteristic of theta waves gave reasonable results, and we determined that there was insufficient training data to improve upon that scale by manual inspection or otherwise.
 Although the length scale was fixed at a level representative of theta waves, we expect that variations in the constant term over time will still reflect ratios in the various types of brain waves.
 In Figures \ref{figure:ictalonset5} and \ref{figure:ictalonset6} it can be seen that sections of the signal with prominent low-frequency components give high values for the extracted feature, and vice-versa.
 In those same figures, it can be seen that the onset of ictal activity generally seems to involve a move from lower-valued LMFT features to higher-valued ones, although perhaps not in a uniform fashion.
 This observation has informed our hypothesis that the performance of DTW will increase when applied to the LMFT features, since it need only discover the relatively simple transition over time from low to high value, rather than an intricate series of ups and downs associated with the raw eeg signals.

\subsubsection{Confirmatory Results}

Having decided upon a covariance function family and a setting for the various hyperparameters in the exploratory analysis, we proceed to extract features from every channel of every sequence.
 We then employ the validation process as described in Section \ref{section:eegmethodology}.

The confusion matrices for the 3 proposed datasets - raw data, LMFT features and the concatenation of the two - are given in Table \ref{table:eegconfusion}.
 It can be seen that 1NN using DTW for classifying sequences of nonictal eeg activity vs the onset of ictal activity using the raw data is ineffective.
 Indeed, the true label and the predicted label are entirely independent.
 Upon inspection, it seems that 17/19 of the true positive and 15/19 of the true negative validation sequences were matched to two of the training sequences.
 Interestingly, although one of those training sequences was true positive and one true negative, there was no correlation to the label of the validation sequences to which they were matched.
 It is not clear what the cause of this strong preference for certain training sequences was, but the lack of correlation reveals that the raw data are not useful for input directly into a classifier.
 
Similarly, when the raw data and the extracted features were concatenated, 34/38 of the validation sequences were matched to two of the training sequences.
 These two sequences were both negative, and were both different from the two popular sequences from the 1NN with DTW on only the raw data.
 We had expected that the combined information of the raw data and the extracted features would be \emph{more} informative for a classification algorithm, but this did not turn out to be the case.

1NN with DTW on only the LMFT features performed better.
 The gains were modest, giving an accuracy, precision and recall of only 0.66, 0.75 and 0.47 respectively. 
 Still, the intention of the experiment was to show that the LMFT extracted features could be useful for a later classification step, and so these results support our hypothesis.
 We remind the reader that there exist opportunities for training over hyperparamters with larger datasets, and also that the proposed algorithm accepts arbitrary model families.
 This suggests that many improvements to the proposed method might still be made, even for this particular task of epilepsy detection.

\begin{table}[h!]
  \begin{center}
    \caption{EEG classification confusion matrices}
    \label{table:eegconfusion}
    \begin{tabular}{llll|ll|ll}
        &   & \multicolumn{6}{c}{\textbf{Predicted}} \\
        &   & \multicolumn{2}{c}{\textbf{Raw Data}} & \multicolumn{2}{c}{\textbf{LMFT}} & \multicolumn{2}{c}{\textbf{Both}} \\
        &   & -    & +    & -    & +    & -    & +    \\
      \multirow{2}{*}{\textbf{True}}
        & - & 14   & 5    & 16   & 3    & 0    & 19   \\
        & + & 14   & 5    & 10   & 9    & 0    & 19
    \end{tabular}
  \end{center}
\end{table}

%TODO We should go and do a post-hoc analysis on why the misclassified ones were misclassified by viewing the extracted features and seeing what the exemplar model was.


==> sections/symbols/symbols.tex <==
\phantomsection 
\vspace*{1in} 
\addcontentsline{toc}{section}{}
\begin{center}
  \vspace*{0.55in}
 \textbf{}
\end{center}
\vspace{0.25 in}

\pagenumbering{roman}
\setcounter{page}{9}

\begin{tabular}{l l}

$a$ 			& 	specific activity\\
$C$ 			&	component concentration, $\mathrm{mol^1}$$\mathrm{m^{-3}}$\\
$C_P$			&	heat capacity, $\mathrm{J^1}$$\mathrm{mol^{-1}}$$\mathrm{K^{-1}}$\\
$d$			&	diameter, $\mathrm{m}$\\
$\mathcal{D}$	& 	component diffusivity, $\mathrm{m^{2}}$$\mathrm{s^{-1}}$\\
$d_b$ 		&	bubble diameter, $\mathrm{m}$\\
$d_{b0}$ 		&	initial bubble diameter, $\mathrm{m}$\\
$d_t$ 			&	internal reactor diameter, $\mathrm{m}$\\
$E_A$			&	activation energy, $\mathrm{J^{1}}$$\mathrm{mol{-1}}$\\
$f$ 			&	volume of solids per volume of bed\\
$g$ 			&	gravitational constant, $\mathrm{m^{1}}$$\mathrm{s^{-2}}$\\
$H_r$			&	heat of reaction, $\mathrm{J^1}$$\mathrm{mol^{-1}}$\\
$HCl$			&	hydrogen chloride\\
$K$			&	gas interchange coefficient, $\mathrm{s^{-1}}$\\
$k$			&	reaction rate constant, $\mathrm{mol^{1}}$$\mathrm{kg_{cat}^{-1}}$$\mathrm{Pa^{-1.003}}$ for Fe\\
			&	$\mathrm{mol^{1}}$$\mathrm{kg_{cat}^{-1}}$$\mathrm{Pa^{-1.086}}$ for Cu\\
$k_1$			&	Boltzmann constant, $\mathrm{J^1}$$\mathrm{molecule^{-1}}$$\mathrm{K^{-1}}$\\
$K$			&	gas interchange coefficient, $\mathrm{s^{-1}}$\\
$K_p$ 		&	equilibrium constant\\ 
$K_r$			&	reaction rate constant (first order reaction), $\mathrm{s^{-1}}$\\
\end{tabular}
\vspace{0.55 in}

\begin{tabular}{l l}
$M$			& 	molar mass $\mathrm{g^1}$$\mathrm{mol^{-1}}$\\
$\dot{m}$		&	mass flow rate, $\mathrm{kg^1}$$\mathrm{s^{-1}}$\\
$\dot{n}$		&	molar flow rate, $\mathrm{mol^1}$$\mathrm{s^{-1}}$\\
$N_{or}$		&	orifice density, $\mathrm{m^{-2}}$\\
$p$ 			&	partial pressure, $\mathrm{Pa}$\\
$p_{atm}$		&	atmospheric pressure, $\mathrm{Pa}$\\
$Q$			&	heat transfer, $\mathrm{W}$\\
$Q_p$		&	reaction quotient\\
$R$ 			&	ideal gas constant, $\mathrm{J^1}$$\mathrm{mol^{-1}}$$\mathrm{K^{-1}}$\\
$r$ 			& 	reaction rate, $\mathrm{mol^1}$$\mathrm{s^{-1}}$$\mathrm{kg_{cat}^{-1}}$\\
$Si$			&	silicon\\
$STC$			&	silicon tetrachloride\\
$T$ 			&	temperature, $\mathrm{K}$\\
$\dot{T}$		&	temperature change per meter, $\mathrm{K^{1}}$$\mathrm{m^{-1}}$\\
$T_b$			&	normal boiling temperature, $\mathrm{K}$\\
$TCS$			&	trichlorosilane\\
$u_0$			&	superficial velocity, $\mathrm{m^{1}}$$\mathrm{s^{-1}}$\\
$u_b$ 		&	average bubble velocity, $\mathrm{m^{1}}$$\mathrm{s^{-1}}$\\
$u_{br}$		&	single bubble rise, $\mathrm{m^{1}}$$\mathrm{s^{-1}}$\\
$u_{mf}$		&	minimum fluidization velocity, $\mathrm{m^{1}}$$\mathrm{s^{-1}}$\\
$v$ 			&	stoichiometric coefficient\\
$V_b$			&	liquid molar volume at normal boiling point, $\mathrm{cm^3}$$\mathrm{mol^{-1}}$\\
$x$ 			&	exponential power\\
$Y$			&	yield, \% \\
$z$			&	reactor height, $\mathrm{m}$
\end{tabular}
\vspace{1 in}


\textit{\textbf{Greek letters}}
\vspace{0.25 in}

\begin{tabular}{l l}
$\alpha$		&	volume of wake over volume of bubble\\
$\Delta$		&	change in\\
$\delta$		&	bed fraction in bubbles\\
$\delta_A$		&	polar parameter\\
$\epsilon$		&	fraction of voids in the bed\\
$\varepsilon$	&	energy parameter for interaction between molecules, $\mathrm{kg^1}$$\mathrm{m^2}$$\mathrm{s^{-2}}$$\mathrm{molecule^{-1}}$\\ 
$\gamma$		&	fractional weight of catalyst\\
$\lambda$		& 	average duration of bubble life, $\mathrm{s}$\\
$\mu_p$		&	dipole moment, $\mathrm{debye}$\\
$\Omega_D$		&	diffusion collision integral\\
$\varphi$		&	parameter unique to Werther \cite{r11} correlation\\
$\rho$		&	density, $\mathrm{kg^{1}}$$\mathrm{m^{-3}}$\\
$\sigma$		&	characteristic length, {\AA}\\		
$\vartheta$		&	parameter unique to Werther \cite{r11} correlation\\
\end{tabular}
\vspace{0.55 in}
\clearpage

\textit{\textbf{Subscripts}}
\vspace{0.25 in}

\begin{tabular}{l l}
$A$			& 	component A (first order reaction)\\
$AVG$		&	average\\
$b$			&	bubble phase\\
$BULK$		&	bulk phase\\
$c$			&	cloud phase\\
$CHLOR$		&	chlorination reaction,  \textit{see Eq.\ref{eq:chlorination}}\\
$Cu_xSi_y$		&	copper catalyzed reaction\\
$DIST$		&	distributor\\
$e$			&	emulsion phase\\
$Fe_xSi_y$		&	iron catalyzed reaction\\
$HEATER$		& 	process gas heater\\
$HYDR$		&	hydrochlorination reaction, \textit{see Eq.\ref{eq:hydrochlorination}}\\
$i$			&	component ($STC$, $H_2$, $TCS$)\\
$IN$			&	actual feed stream\\
$mf$			& 	minimum fluidization\\
$mg$			& 	metallurgical grade silicon\\
$n$			&	n$^{th}$ number (in an experimental set)\\
$N$			&	total number (of an experimental set)\\
$OUT$		&	product stream\\
$RX$			&	reaction section of the reactor\\
$Si$			&	silicon\\
$STC$			&	silicon tetrachloride\\
$TCS$			&	trichlorosilane\\
$w$			&	wake phase\\
$0$			&	model initialization value\\
\end{tabular}


